TrapSIMD: SIMD-Aware Compiler Optimization for 2D Trapped-Ion Quantum Machines

Modular trapped-ion (TI) architectures offer a scalable quantum computing (QC) platform, with native transport behaviors that closely resemble the Single Instruction Multiple Data (SIMD) paradigm. We present FluxTrap, a SIMD-aware compiler framework that establishes a hardware-software co-design interface for TI systems. FluxTrap introduces a novel abstraction that unifies SIMD-style instructions -- including segmented intra-trap shift SIMD (S3) and global junction transfer SIMD (JT-SIMD) operations -- with a SIMD-enriched architectural graph, capturing key features such as transport synchronization, gate-zone locality, and topological constraints. It applies two passes -- SIMD aggregation and scheduling -- to coordinate grouped ion transport and gate execution within architectural constraints. On NISQ benchmarks, FluxTrap reduces execution time by up to $3.82 \times$ and improves fidelity by several orders of magnitude. It also scales to fault-tolerant workloads under diverse hardware configurations, providing feedback for future TI hardware design.

==> 01_introduction_v1.tex <==
\section{Introduction}
\label{sect:introduction}

\begin{figure*}[bp!]
        \centering
        \includegraphics[width=0.95\linewidth]{fig/intro_hardware.pdf}
        
        \caption{Scalable QCCD architecture combining H2 trap design with four-leg junctions and its hardware constraints.}
        \label{fig:intro_hardware}
\end{figure*}

Quantum computing (QC) has experienced rapid advancements, with multiple platforms achieving significant breakthroughs in recent years~\cite{arute2019quantum, huang2020superconducting, bravyi2022future, bruzewicz2019trapped, chen2023benchmarking, kok2007linear, bourassa2021blueprint, bluvstein2024logical, wurtz2023aquila}. With each platform offering distinct advantages and continuing to advance, competition among them is expected to persist. Among them, trapped ion (TI) systems, which was proposed as one of the original platforms for quantum computing around 30 years ago \cite{cirac1995quantum}, have remained a leading candidate for quantum processors, due to its long coherence time of qubits \cite{??} and high fidelity of various operations \cite{03_02_new_ion_hardware}.

Traditional trapped ion quantum processors typically feature a 1D geometry with full connectivity between ions in the trap. This architecture faces scaling challenges, as the realization of full connectivity leads to significant control overhead as the number of ions increases \cite{malinowski2023wire}. A promising solution to this limitation is the scalable quantum charge-coupled device (QCCD) architecture, which connects multiple short 1D traps into a 2D grid with junctions between them \cite{02_25_grid_ion_hardware}. Furthermore, recent advancements in achieving high-fidelity ion transportation within each 1D trap \cite{?} have reduced the need for full connectivity, allowing the control overhead to be alleviated.

We base our work on the combination of latest hardware technologies of TI systems. For 1D traps, we adopt the trap design of the H2 hardware of Quantinuum \cite{03_02_new_ion_hardware}. It divides a trap into interleaved gate zones and auxiliary zones, with fast and high-fidelity supported for qubits in the gate zones,  fast and high-fidelity ion transportation, including ion shift and ion swap, supported within the whole trap. For 2D junctions, we adopt the four-leg junction that has been recently realized by Quantinuum \cite{02_25_grid_ion_hardware}. It can connect four 1D traps with its four legs, allowing ion transportation, including ion shift and ion swap, between the edge qubits of the four traps. This combination enables a modular grid structure, facilitating the scalability of future TI processors.



However, these new hardware features brings new challenges for program compilation, which cannot be resolved by existing compilers [?][?][?]. First, none of existing frameworks can fully utilize the flexibility enabled by the latest hardware: compilers of traditional TI systems [?][?] do not support native ion swap operation. In a 1D trap, they utilize SWAP gates to swap qubit data, which results in lower operation fidelity, as the fidelity of a SWAP gate (equivalent to three CNOT gates) is much lower than that of ion transportation. Among 1D traps, they do not support native in-place ion swap operation. An ion-swap would be translated to multiple ion shifts, which incurs unnecessary overhead. Compilers developed for other gate-based platforms cannot achieve this either. For example, compilers for superconducting platforms [?][?] cannot leverage the ability of concurrently shifting multiple ions in TI systems, while compilers for neutral atom platforms [?][?] are not aware of the 1D constraints of each trap.

Second, the performance distinction between different operations introduces heterogeneity to the computing system. Specifically, ion transportation operations are slower than gate operations, with inter-trap transportation being slower than intra-trap transportation, and with ion swap being slower than ion shift. In order to achieve computation efficiency, it is essential to carefully interleave different operations to minimize their wait time for each other's completion. However, this multi-hierarchy performance cannot be captured by a simple abstraction such as the circuit depth in traditional gate-based compilers. Rather, it requires a more fined-grained coordination that takes the fidelity and latency of different operations into account.

Third, these latest hardware technologies come with their own constraints. In a 1D trap, gate operations can only be conducted in the gate zones, while the auxiliary zones can only be used to hold ions. This restricts the computation resource and can cause server contention for gates zones if not carefully optimized. Among 1D traps, operations can only be performed globally across all junctions. That is, while each ion can choose to \emph{stay-or-move} during a global transportation, inter-trap transportation is not allowed to be conducted concurrently with intra-trap transportation. Furthermore, all moved ions must be transported by the same type of operation, either \emph{shift-or-swap}, along the same direction, e.g., all from the left leg to the bottom leg. 
% This constraint is unique for the latest four-leg junction technology, which requires additional awareness by the compilation optimization.

\begin{figure*}[t!]
        \centering
        \includegraphics[width=0.9\linewidth]{fig/intro_flow.pdf}
        
        \caption{Overall flow of our compiler.}
        \label{fig:intro_flow}
\end{figure*}

To overcome these challenges, we identify three aspects that require novel techniques.
% propose the following techniques to facilitate an efficient compilation.
(1) A new instruction set architecture (ISA) is required to capture the features of native operations on the latest TI hardware, so that parallel operations can be recognized easily without converting to other instructions, such as converting ion swap to shift operations in the old TI ISA or to sequential SWAP gates in the superconducting ISA. (2) A performance-aware scheduler is needed to compactly interleave different operations, so that the wait time of distinct operations can be minimized without incurring local or global conflicts, such as conflicted intra-trap moving targets or inter-trap moving directions. (3) An optimized router is necessary to coordinate different types and directions of ion transportation. This should on one hand strategically minimize the moving distance of each ion, and on the other hand prevent congestion caused by the contention for limited gate zones in the 1D traps.

To this end, we propose a compilation framework for this scalable TI architecture. We first propose an \textbf{IonShiftOrSwap (ISOS) ISA} to support native TI operations with four primary instructions: \texttt{intra\_shift(src, dst)}, \texttt{intra\_swap(q1, q2)}, \texttt{global\_inter} \texttt{\_shift(ion\_set)} and \texttt{global\_inter\_swap(ion\_set)}. Other instructions include single-qubit (1Q) gates, two-qubit (2Q) gates and measurements, as in common gate-based ISAs. We further specify the resource condition of each instruction to facilitate the validation and conflict detection of different instructions in the scheduling and routing passes. This ISA opens up a broader optimization space for the latest TI architecture, enabling full exploitation of its flexibility while ensuring the compliance to its constraints.

We then propose a \textbf{simulation-based scheduler} to accommodate the distinction between different types of operations. Specifically, we realize a \textbf{discrete event simulator} that simulates the instruction execution in a fine-grained manner, indicating accumulated operation latency on each possible ion location and detecting conflicts between scheduled instructions. 
% Based on the simulator, our scheduler tracks the accumulated latency of each possible ion position, including computation zones and auxiliary zones, searching for the next suitable operation with a priority of local operations over global ones. 
Based on the simulator, our scheduler iteratively \textbf{finds concurrent transportation} according to program demand, prioritizing the search for local operations over global ones. Specifically, it maintains an instruction table for concurrent operations and a directed acyclic graph (DAG) that represents required gates by the program. 
% It dynamically updates the instruction table and the DAG by adding new concurrent operations until exhaustion, then iteratively pushing the instructions (completely or partially) to the simulator and removing the executable gates from the DAG. In this way, it can maximize the parallelism between transportation, thereby enhancing the efficiency and resource utilization of the compilation.
% By iteratively adding operations to the instruction table until exhaustion, pushing instructions (completely or partially) to the simulator and removing executable gates from the DAG, it maximizes the parallelism between transportation, thereby enhancing the efficiency and resource utilization.
By dynamically managing empty locations required and left by moved ions, iteratively pushing concurrent instructions (completely or partially) to the simulator and updating the DAG, it enables grouped ion transportation, thereby enhancing program efficiency.

Lastly, we propose a \textbf{heuristic router} with a carefully designed cost function to further optimize the transportation trajectory of each ion. This router not only aims to minimize the routing distance of ion transportation, but also to prevent congestion by mitigating the contention of ions for the limited gate zones. This is achieved by incorporating two terms into the heuristic function, with one term punishing the distance between qubits involved in near-future gates and the other term punishing the distance from qubits to available gate zones. In contrast to a route-then-detect-congestion strategy in previous TI compilers [?][?], this router will be used by the scheduler for a step-by-step operation search in each scheduling iteration. This enables a complete elimination of gate zone contention, thereby preventing congestion more efficiently. 




==> 01_introduction_v2.tex <==
\section{Introduction}
\label{sect:introduction}

\begin{figure*}[bp!]
        \centering
        \includegraphics[width=0.98\linewidth]{fig/intro_hardware.pdf}
        
        \caption{TI architecture combining 1D traps with 2D junctions, with gate zones and auxiliary zones in yellow and gray.}
        \label{fig:intro_hardware}
\end{figure*}

Quantum computing (QC) has experienced rapid advancements, with multiple platforms achieving significant breakthroughs in recent years~\cite{arute2019quantum, huang2020superconducting, bravyi2022future, bruzewicz2019trapped, chen2023benchmarking, kok2007linear, bourassa2021blueprint, bluvstein2024logical, wurtz2023aquila}. With each platform offering distinct advantages and continuing to advance, competition among them is expected to persist. Among them, trapped ion (TI) systems, which was proposed as one of the original platforms for quantum computing around 30 years ago \cite{cirac1995quantum}, have remained a leading candidate for quantum processors, due to its long coherence time of qubits \cite{??} and high fidelity of various operations \cite{03_02_new_ion_hardware}.


This paper bases on the combination of latest hardware technologies of Quantinuum -- a leading competitor in TI systems.
In their latest H2 processor \cite{03_02_new_ion_hardware}, \textbf{1D ion traps} have been realized with fast and high-fidelity ion transportation within each trap, including ion shift (i.e., moving an ion to an empty location) and ion swap (i.e., switching the locations of two neighboring ions). Recently, Quantinuum has also proposed a novel \textbf{2D junction} \cite{02_25_grid_ion_hardware} to connect 1D ion traps into a 2D grid, thereby overcoming the scalability limitations of 1D ion traps, including the increasing control and calibration overhead as the number of ion increases \cite{malinowski2023wire}[?][?], with a modular architecture.

As shown in Fig.~\ref{fig:intro_hardware}, in Quantinuum's architecture, each 1D trap is divided into interleaved gate zones (depicted in yellow) and auxiliary zones (depicted in gray), with single-qubit (1Q) gates supported in gate zones and two-qubit (2Q) gates supported between qubits in gate zones and their neighbors (i.e., moving the neighbor into the gate zone, implementing the gate and moving back). Each junction can connect four 1D traps with its four legs, with transportation allowed between the ion locations on the edge of the connected 1D traps, including ion shifts and ion swaps. 


% We base our work on the combination of latest hardware technologies of TI systems. For 1D traps, we adopt the trap design of the H2 hardware of Quantinuum \cite{03_02_new_ion_hardware}. It divides a trap into interleaved gate zones and auxiliary zones, with fast and high-fidelity supported for qubits in the gate zones,  fast and high-fidelity ion transportation, including ion shift and ion swap, supported within the whole trap. For 2D junctions, we adopt the four-leg junction that has been recently realized by Quantinuum \cite{02_25_grid_ion_hardware}. It can connect four 1D traps with its four legs, allowing ion transportation, including ion shift and ion swap, between the edge qubits of the four traps. This combination enables a modular grid structure, facilitating the scalability of future TI processors.



However, this emerging architecture brings new challenges for compilation, which cannot be resolved by existing compilers [?][?][?]. First, none of existing frameworks can fully utilize the flexibility enabled by the latest hardware: traditional TI compilers [?][?] do not support native ion swap operation. In a 1D trap, they utilize SWAP gates to swap qubit data, resulting in lower operation fidelity, as the fidelity of SWAP gates is much lower than ion transportation. Among 1D traps, each native in-place ion swap operation would be translated to multiple ion shifts, incurring unnecessary overhead. Compilers for other gate-based platforms are also suboptimal: compilers for superconducting platforms [?][?] cannot leverage the ability of concurrently shifting multiple ions in TI systems, while compilers for neutral atom platforms [?][?] are not aware of the 1D geometry of ion traps.

Second, the performance distinction between different operations introduces heterogeneity to the computing system. Specifically, ion transportation is slower than gate operations, with inter-trap transportation being slower than intra-trap transportation, and ion swap being slower than ion shift. In order to achieve computation efficiency, it is essential to carefully interleave different operations to minimize their wait time. However, this multi-hierarchy performance cannot be captured by a simple abstraction such as the circuit depth in traditional gate-based compilers. Rather, it requires a fined-grained coordination taking fidelity and latency of different operations into account.

Third, this architecture come with its own hardware constraints. In a 1D trap, gate operations can only be conducted in the gate zones, while the auxiliary zones can only be used to hold ions. This restricts the computation resource and can cause server contention for gates zones if not carefully optimized. Among 1D traps, operations can only be performed globally across all junctions. That is, while each ion can choose to \emph{stay-or-move} during a global transportation, inter-trap transportation is not allowed to be conducted concurrently with intra-trap transportation (Fig.~\ref{fig:intro_hardware}(a)). Furthermore, all moved ions must be transported by the same type of operation (Fig.~\ref{fig:intro_hardware}(b)), either \emph{shift-or-swap}, along the same direction, e.g., all from the left leg to the bottom leg (Fig.~\ref{fig:intro_hardware}(c)). 
% This constraint is unique for the latest four-leg junction technology, which requires additional awareness by the compilation optimization.

\begin{figure*}[t!]
        \centering
        \includegraphics[width=0.96\linewidth]{fig/intro_flow.pdf}
        
        \caption{Overall flow of our compiler.}
        \label{fig:intro_flow}
\end{figure*}

To overcome these challenges, we identify three aspects that require novel techniques.
% propose the following techniques to facilitate an efficient compilation.
(1) A new instruction set architecture (ISA) is required to capture the features of native operations on the latest TI hardware, so that parallel operations can be recognized easily without converting to other instructions. (2) A performance-aware scheduler is needed to compactly interleave different operations, so that the wait time of distinct operations can be minimized without incurring conflicts such as conflicted intra-trap moving targets or inter-trap moving directions. (3) An optimized router is necessary to coordinate different types and directions of ion transportation. This should on one hand strategically minimize the moving distance of each ion, and on the other hand prevent congestion caused by the contention for limited gate zones in the 1D traps.

To this end, we propose a compilation framework for this scalable TI architecture. We first propose an \textbf{IonShiftOrSwap (ISOS) ISA} to support native TI operations with four primary instructions: \texttt{intra\_shift(src, dst)}, \texttt{intra\_swap(q1, q2)}, \texttt{global\_inter} \texttt{\_shift(ion\_set)} and \texttt{global\_inter\_swap(ion\_set)}. Other instructions include single-qubit (1Q) gates, two-qubit (2Q) gates and measurements, as in common gate-based ISAs. We further specify the resource condition of each instruction to facilitate the validation and conflict detection of different instructions in the scheduling and routing passes. This ISA opens up a broader optimization space for the latest TI architecture, enabling full exploitation of its flexibility while ensuring the compliance to its constraints.

We then propose a \textbf{simulator-based scheduler} to accommodate the distinction between different operations. We realize a \textbf{discrete event simulator} that simulates the instruction execution in a fine-grained manner, indicating accumulated operation latency on each ion location and detecting conflicts between scheduled instructions. 
% Based on the simulator, our scheduler tracks the accumulated latency of each possible ion position, including computation zones and auxiliary zones, searching for the next suitable operation with a priority of local operations over global ones. 
Based on it, our scheduler iteratively \textbf{finds concurrent transportation} in the program, prioritizing the search for local operations over global ones. Specifically, it maintains an instruction table for concurrent operations and a directed acyclic graph (DAG) representing gates required by the program. 
% It dynamically updates the instruction table and the DAG by adding new concurrent operations until exhaustion, then iteratively pushing the instructions (completely or partially) to the simulator and removing the executable gates from the DAG. In this way, it can maximize the parallelism between transportation, thereby enhancing the efficiency and resource utilization of the compilation.
% By iteratively adding operations to the instruction table until exhaustion, pushing instructions (completely or partially) to the simulator and removing executable gates from the DAG, it maximizes the parallelism between transportation, thereby enhancing the efficiency and resource utilization.
By dynamically managing empty locations targeted and left by moved ions, iteratively pushing concurrent instructions (completely or partially) to the simulator and updating the DAG, it enables grouped ion transportation, thereby enhancing program efficiency.

Lastly, we propose a \textbf{heuristic router} with a carefully designed cost function to further optimize the transportation trajectory of each ion. This router not only aims to minimize the routing distance of ion transportation, but also to prevent congestion by mitigating the contention of ions for the limited gate zones. This is achieved by incorporating two terms into the heuristic function, with one term punishing the distance between qubits involved in near-future gates and the other term punishing the distance from qubits to available gate zones. In contrast to a route-then-detect-congestion strategy in previous TI compilers [?][?], this router will be used by the scheduler for a step-by-step operation search in each scheduling iteration. This enables a complete elimination of gate zone contention, thereby preventing congestion more efficiently. 

Our contributions in this paper can be summarized as below.
\begin{itemize}
    \item We propose a novel ISA, IonShiftOrSwap, to capture the features of the native operation set on the emerging TI architecture.
    \item We employ a fine-grained scheduler based on a discrete event simulator to accommodate the distinction in latency between different operations.
    \item This scheduler is integrated with a carefully designed heuristic router to minimize the ion transportation while avoiding congestion caused by the contention of gate zones.
    \item Through a comprehensive evaluation, we demonstrate that the compiler with these novel techniques \todo{improves the execution time by a factor of xxx and improves the fidelity by a factor of xxx} 
\end{itemize}




==> 02_introduction_new.tex <==
Quantum computing (QC) has experienced rapid advancements, with multiple platforms achieving significant breakthroughs in recent years~\cite{arute2019quantum, huang2020superconducting, bravyi2022future, bruzewicz2019trapped, chen2023benchmarking, kok2007linear, bourassa2021blueprint, bluvstein2024logical, wurtz2023aquila}. As each platform offers distinct advantages and continues to advance, competition among them is expected to persist. Among them, trapped ion (TI) systems, which was proposed as one of the original platforms for quantum computing around 30 years ago \cite{cirac1995quantum}, have remained a leading candidate for quantum processors, due to its long coherence time of qubits \cite{03_02_qccd_old_version} and high fidelity of various operations \cite{03_02_new_ion_hardware}.

This paper builds upon recent architectural trends in trapped-ion (TI) quantum computing, particularly the transition toward modular and scalable designs. A leading approach is the \emph{Quantum Charge-Coupled Device (QCCD)} architecture, which integrates high-fidelity \textbf{1D ion traps}—where ions can be shifted or swapped along linear segments—with \textbf{2D junctions} that allow ions to move between traps. This structure forms a scalable 2D grid, enabling flexible routing and interaction across physically distinct regions~\cite{02_25_grid_ion_hardware, 02_26_modular_ion_trap, x_junction0}. As a representative implementation, we refer to Quantinuum’s modular TI processor~\cite{03_02_new_ion_hardware, 02_25_grid_ion_hardware}, which embodies the broader direction of TI hardware development~\cite{malinowski2023wire, 03_02_qccd_old_version}.

To appreciate the architectural and performance implications of this architecture, it is useful to contrast it with more traditional superconducting systems\cite{superconducting_0, superconducting_1}. In superconducting architectures, qubits are fixed on a 2D grid and interact through nearest-neighbor couplings governed by a static coupling graph. By contrast, trapped-ion systems leverage \emph{mobile qubits}: ions that can be actively shuttled within and across trap segments. This mobility offers greater connectivity and layout flexibility, but also introduces new challenges for compilation and control.

In QCCD systems, these challenges arise from several physical constraints. First, 1D ion traps are spatially divided into \emph{gate zones} (where quantum gates can be performed) and \emph{auxiliary zones} (which serve as temporary storage)\cite{02_25_ion_CCD, 03_02_new_ion_hardware}. Second, distinct operation types—including gate execution, intra-trap transport, and inter-trap transport—exhibit significantly different latencies and fidelities\cite{03_03_ion_operation_time}. Third, to reduce laser control overhead and simplify timing coordination, inter-trap transport across 2D junctions is performed globally in a coordinated manner: all participating ions must move in the same direction and use the same transport primitive (e.g., shift or swap), and such operations are mutually exclusive with intra-trap movements.

Interestingly, the 2D global synchronization constraint mirrors the behavior of \textbf{Single Instruction Multiple Data (SIMD)} execution in classical computing\cite{classical_simd}, where a single control signal triggers uniform operations across multiple data elements. In trapped-ion systems, inter-trap transport adopts a similar model: a single instruction (e.g., “shift right”) governs movement across the entire 2D system in that round. Even within individual traps, although the hardware allows flexible ion shuttling, performance is improved by grouping shifts into coordinated patterns—such as moving multiple ions toward a shared gate zone—which again reflects a SIMD-style behavior.

==> 02_introduction_v3.tex <==
\section{Introduction}
\label{sect:introduction}
\todo{fix into SIMD contribution}
% \begin{figure*}[!t]
% %\begin{figure*}[bp!] [h!]
%         \centering
%         \includegraphics[width=0.98\linewidth]{fig/intro_hardware.pdf}
        
%         \caption{TI architecture combining 1D traps with 2D junctions, with gate zones and auxiliary zones in yellow and gray.}
%         \label{fig:intro_hardware}
% \end{figure*}

Quantum computing (QC) has experienced rapid advancements, with multiple platforms achieving significant breakthroughs in recent years~\cite{arute2019quantum, huang2020superconducting, bravyi2022future, bruzewicz2019trapped, chen2023benchmarking, kok2007linear, bourassa2021blueprint, bluvstein2024logical, wurtz2023aquila}. As each platform offers distinct advantages and continues to advance, competition among them is expected to persist. Among them, trapped ion (TI) systems, which was proposed as one of the original platforms for quantum computing around 30 years ago \cite{cirac1995quantum}, have remained a leading candidate for quantum processors, due to its long coherence time of qubits \cite{03_02_qccd_old_version} and high fidelity of various operations \cite{03_02_new_ion_hardware}.

This paper builds upon recent architectural trends in trapped-ion (TI) quantum computing systems, particularly the shift toward modular and scalable designs. A common approach is to use high-fidelity \textbf{1D ion traps} that support fast ion transport operations, such as ion shift (moving an ion to an empty location) and ion swap (exchanging two neighboring ions). To address the growing control overhead in large-scale 1D chains, a \textbf{2D junction architecture} has been proposed in several platforms, enabling the interconnection of multiple 1D traps into a 2D grid structure for enhanced scalability. 
Without loss of generality, we use the quantum processor developed by Quantinuum—a leading company in TI quantum hardware—as a concrete example to illustrate these architectural features \cite{03_02_new_ion_hardware, 02_25_grid_ion_hardware}. Their implementation reflects the broader direction of the TI community and exemplifies the practical realization of such modular architectures \cite{malinowski2023wire, 02_26_modular_ion_trap, 03_02_qccd_old_version}.


%This paper is based on the combination of the latest hardware technologies of Quantinuum, a leading competitor in TI systems. In their latest H2 processor \cite{03_02_new_ion_hardware}, \textbf{1D ion traps} have been realized with fast and high-fidelity ion transportation within each trap, including ion shift (i.e., moving an ion to an empty location) and ion swap (i.e., switching the locations of two neighboring ions). Recently, Quantinuum has also proposed a novel \textbf{2D junction} \cite{02_25_grid_ion_hardware} to connect 1D ion traps into a 2D grid, thereby overcoming the scalability limitations of 1D ion traps, including the increasing control and calibration overhead as the number of ion increases \cite{malinowski2023wire}[?][?], with a modular architecture.

As shown in Fig.~\ref{fig:intro_hardware}, in Quantinuum's architecture~\cite{}, each 1D trap is divided into interleaved gate zones (depicted in yellow) and auxiliary zones (depicted in gray), with single-qubit (1Q) gates supported in gate zones and two-qubit (2Q) gates supported between qubits in gate zones and their neighbors (i.e., moving the neighbor into the gate zone, implementing the gate and moving back). Each junction can connect four 1D traps with its four legs, with transportation allowed between the ion locations on the edge of the connected 1D traps, including ion shifts and ion swaps. 


% We base our work on the combination of latest hardware technologies of TI systems. For 1D traps, we adopt the trap design of the H2 hardware of Quantinuum \cite{03_02_new_ion_hardware}. It divides a trap into interleaved gate zones and auxiliary zones, with fast and high-fidelity supported for qubits in the gate zones,  fast and high-fidelity ion transportation, including ion shift and ion swap, supported within the whole trap. For 2D junctions, we adopt the four-leg junction that has been recently realized by Quantinuum \cite{02_25_grid_ion_hardware}. It can connect four 1D traps with its four legs, allowing ion transportation, including ion shift and ion swap, between the edge qubits of the four traps. This combination enables a modular grid structure, facilitating the scalability of future TI processors.



However, this emerging architecture brings new challenges for compilation, which cannot be resolved by existing compilers. First, this architecture comes with its own hardware constraints. Among 1D traps, operations can only be performed globally across all junctions. That is, while each ion can choose to \emph{stay-or-move} during a global transportation, inter-trap transportation is not allowed to be conducted concurrently with intra-trap transportation (Fig.~\ref{fig:intro_hardware}(a)). Furthermore, all moved ions must be transported by the same type of operation (Fig.~\ref{fig:intro_hardware}(b)), either \emph{shift-or-swap}, along the same direction, e.g., all from the left leg to the bottom leg (Fig.~\ref{fig:intro_hardware}(c)). 
% This constraint is unique for the latest four-leg junction technology, which requires additional awareness by the compilation optimization.

Second, in each 1D trap, gate operations can only be conducted in the gate zones, while the auxiliary zones can only be used to hold ions. This restricts the computation resource and can cause severe contention for gates zones if not carefully optimized. Existing TI compilers [?] routes ions by identifying a suitable path, lacking coordination between different ions and different types of transportation. This can easily lead to congestion, due to both the conflicts between different paths and the contention for the limited gate zones. 
\begin{figure*}[h!]
        \centering
        \includegraphics[width=\linewidth, trim=0in 0in 0.2in 0in, clip]{fig/intro.pdf}
        
        \caption{Overall flow of our compiler.}
        \label{fig:intro_flow}
\end{figure*}
% Third, none of existing frameworks can fully utilize the flexibility enabled by the latest hardware: traditional TI compilers [?][?] do not support native ion swap operation. In a 1D trap, they utilize SWAP gates to swap qubit data, resulting in lower operation fidelity, as the fidelity of SWAP gates is much lower than ion transportation. Among 1D traps, each native in-place ion swap operation would be translated to multiple ion shifts, incurring unnecessary overhead. Compilers for other gate-based platforms are also suboptimal: compilers for superconducting platforms [?][?] cannot leverage the ability of concurrently shifting multiple ions in TI systems, while compilers for neutral atom platforms [?][?] are not aware of the 1D geometry of ion traps.

Third, the performance distinction between different operations introduces heterogeneity to the computing system. Specifically, ion transportation is slower than gate operations, with inter-trap transportation being slower than intra-trap transportation, and ion swap being slower than ion shift. In order to achieve computation efficiency, it is essential to carefully interleave different operations to minimize their wait time. However, this multi-hierarchy performance cannot be captured by a simple abstraction such as the circuit depth in traditional gate-based compilers. Rather, it requires a fined-grained coordination taking fidelity and latency of different operations into account.\todo{may add quantitative time information at the order-of-magnitude level}



% \begin{figure*}[t!]
%         \centering
%         \includegraphics[width=0.96\linewidth]{fig/intro_flow2.pdf}
        
%         \caption{Overall flow of our compiler.}
%         \label{fig:intro_flow}
% \end{figure*}


To overcome these challenges, we identify three aspects that require novel techniques.
% propose the following techniques to facilitate an efficient compilation.
(1) A new abstraction of the hardware structure is required to capture the features and constraints of native operations of the latest TI hardware.  (2) A congestion-aware router is necessary to enable efficient transportation while being aware of the difference between gates zones and auxiliary zones.
(3) A latency-aware scheduler is needed to compactly interleave different operations, so that the wait time of distinct operations can be minimized, thereby leading to an efficient compilation.




To this end, we propose an abstraction that we call the \textbf{switchable position graph}. The vertices in this graph stand for possible ion locations, where each location can be occupied by an ion or be empty; the edges represent the neighborhood relations between the locations. To comply with the hardware constraints, edges in the graph are not always active, but switch between several patterns: (1) all intra-trap edges are active while all inter-trap edges are inactive; (2) all intra-trap edges are inactive while inter-trap edges in a certain direction of all junctions are active. Compared to prior work, it changes the description of system status from the view of ions to the view of possible locations. This not only allows an easy integration with existing gate-based compilers, but also lays a foundation for the subsequent  optimizations.


We then propose a \textbf{step-by-step router} with a carefully designed cost function to further optimize the transportation trajectory of each ion. In contrast to previous compilers which first search for end-to-end routing paths and then detect congestion, it implements a more fine-grained search with each transportation only taking a single step from a location to its neighborhood, thereby naturally preventing congestion and allowing more flexibility for routing. The heuristic function enables 2Q gates by minimizing both the distance of between corresponding ions and between the ions and gate zones, taking all gates in the near future into account in a weighted manner. It further employs a priority among different 2Q gates to prevent contention for the limited gate zones.


% This router not only aims to minimize the routing distance of ion transportation, but also to prevent congestion by mitigating the contention of ions for the limited gate zones. This is achieved by incorporating two terms into the heuristic function, with one term punishing the distance between qubits involved in near-future gates and the other term punishing the distance from qubits to available gate zones. In contrast to a route-then-detect-congestion strategy in previous TI compilers [?][?], this router will be used by the scheduler for a step-by-step operation search in each scheduling iteration. This enables a complete elimination of gate zone contention, thereby preventing congestion more efficiently. 

Lastly, we propose a \textbf{simulator-based just-in-time (JIT) scheduler} to coordinate the routing of different types of ion transportation. Specifically, it schedules one round of inter-trap transportation after certain rounds of intra-trap transportation, with the number rounds adjusted by an auto-tuned parameter. In each intra-trap round, it schedules multiple concurrent ion shift and ion swap operations, enabling grouped ion shift by carefully managing the empty locations and searching for ion shift before ion swap. The scheduler is JIT in the sense that, after the processing of each instruction by the discrete event simulator, it updates the circuit status, empty locations and the remaining time of incomplete instructions, so that it only needs to hold information about the current status. This updating mechanism makes the scheduling more compact by taking the latency discrepancy between different operations into account, enabling discovery of more optimization opportunities.

% to accommodate the distinction between different operations. We realize a \textbf{discrete event simulator} that simulates the instruction execution in a fine-grained manner, indicating accumulated operation latency on each ion location and detecting conflicts between scheduled instructions. Based on it, our scheduler iteratively \textbf{finds concurrent transportation} in the program, prioritizing the search for local operations over global ones. Specifically, it maintains an instruction table for concurrent operations and a directed acyclic graph (DAG) representing gates required by the program. By dynamically managing empty locations targeted and left by moved ions, iteratively pushing concurrent instructions (completely or partially) to the simulator and updating the DAG, it enables grouped ion transportation, thereby enhancing program efficiency.



Our contributions in this paper can be summarized as below.
\begin{itemize}
    \item We abstract a switchable position graph for TI systems to capture its native operations and hardware constraints. \textcolor{red}{(Jens: rephrase this.)}

    \item We propose a step-by-step router to minimize ion transportation while avoiding congestion caused by the contention of gate zones.
    
    \item We employ a fine-grained JIT scheduler based on a discrete event simulator, providing compact scheduling by enabling grouped ion shift and accommodating the distinction in latency between different operations.
    
    \item Through a comprehensive evaluation, we demonstrate that the compiler with these novel techniques \todo{improves the execution time by a factor of xxx and improves the fidelity by a factor of xxx} 
\end{itemize}




==> 02_introduction_v4.tex <==
\section{Introduction}
\label{sect:introduction}
% \begin{figure*}[!t]
% %\begin{figure*}[bp!] [h!]
%         \centering
%         \includegraphics[width=0.98\linewidth]{fig/intro_hardware.pdf}
        
%         \caption{TI architecture combining 1D traps with 2D junctions, with gate zones and auxiliary zones in yellow and gray.}
%         \label{fig:intro_hardware}
% \end{figure*}

Quantum computing (QC) has experienced rapid advancements, with multiple platforms achieving significant breakthroughs in recent years~\cite{arute2019quantum, huang2020superconducting, bravyi2022future, bruzewicz2019trapped, chen2023benchmarking, kok2007linear, bourassa2021blueprint, bluvstein2024logical, wurtz2023aquila}. As each platform offers distinct advantages and continues to advance, competition among them is expected to persist. Among them, trapped ion (TI) systems, which was proposed as one of the original platforms for quantum computing around 30 years ago \cite{cirac1995quantum}, have remained a leading candidate for quantum processors, due to its long coherence time of qubits \cite{03_02_qccd_old_version} and high fidelity of various operations \cite{03_02_new_ion_hardware}.

One of the leading trapped-ion hardware architectures is the \emph{Quantum Charge-Coupled Device (QCCD)} model, which has become the prevailing design for scalable TI systems~\cite{02_25_grid_ion_hardware, 02_26_modular_ion_trap, x_junction0, malinowski2023wire, 03_02_qccd_old_version} and has been adopted by major vendors such as Quantinuum~\cite{03_02_new_ion_hardware, 02_25_grid_ion_hardware}. QCCD architectures feature high-fidelity \textbf{1D ion traps} that support fast ion transport operations, including ion shifts (moving an ion to an empty site) and ion swaps (exchanging the positions of two adjacent ions). These 1D traps are interconnected via \textbf{2D junctions}—cross-shaped structures that enable ion movement across 1D traps—thereby supporting long-range interactions and enabling modular, scalable system layouts.


%This paper builds upon recent architectural trends in TI QC systems, particularly the transition toward modular and scalable designs. A promising approach is the \emph{Quantum Charge-coupled Device (QCCD)} architecture, which combines high-fidelity \textbf{1D ion traps} that support fast ion movements, such as ion shift (moving an ion to an empty location) and ion swap (exchanging two neighboring ions) with \textbf{2D junctions}. This architecture has been proposed in several platforms \cite{02_25_grid_ion_hardware, 02_26_modular_ion_trap,x_junction0}, enabling the interconnection of multiple 1D traps into a 2D grid structure for enhanced scalability.  Without loss of generality, we use the quantum processor developed by Quantinuum -- a leading company in TI quantum hardware -- as a concrete example to illustrate these architectural features \cite{03_02_new_ion_hardware, 02_25_grid_ion_hardware}. Their implementation reflects the broader direction of the TI community and exemplifies the practical realization of such modular architectures \cite{malinowski2023wire, 02_26_modular_ion_trap, 03_02_qccd_old_version}.


% This paper builds upon recent architectural trends in trapped-ion (TI) QC systems, particularly the transition toward modular and scalable designs. A common approach is to use high-fidelity \textbf{1D ion traps} that support fast ion transport operations, such as ion shift (moving an ion to an empty location) and ion swap (exchanging two neighboring ions). To address the growing control overhead in large-scale 1D chains, a \textbf{2D junction architecture} has been proposed in several platforms, enabling the interconnection of multiple 1D traps into a 2D grid structure for enhanced scalability. 
% Without loss of generality, we use the quantum processor developed by Quantinuum—a leading company in TI quantum hardware—as a concrete example to illustrate these architectural features \cite{03_02_new_ion_hardware, 02_25_grid_ion_hardware}. Their implementation reflects the broader direction of the TI community and exemplifies the practical realization of such modular architectures \cite{malinowski2023wire, 02_26_modular_ion_trap, 03_02_qccd_old_version}.

% To illustrate these architectural features concretely, we reference the design developed by Quantinuum, whose hardware implementation reflects many of the capabilities and constraints present in modern TI systems~\cite{03_02_new_ion_hardware, 02_25_grid_ion_hardware}. 

% To appreciate the performance and architectural implications of QCCD-based trapped-ion systems, it is important to contrast them with more familiar superconducting platforms. 
% To motivate the need for new compilers of TI systems, 
%To achieve optimized compilation for TI systems, it is essential to understand the distinct architectural constraints introduced by the QCCD model. 
Unlike superconducting platforms\cite{superconducting_0, superconducting_1} where qubits are fixed on a 2D grid and interact via static, nearest-neighbor couplings, TI systems utilize qubit transportation for program execution. 
This transport-based architecture enables greater flexibility, but also introduces new physical constraints that compilers must address. In particular: (1) 
% Positions in 1D traps are divided into gates zones and auxiliary zones\cite{02_25_ion_CCD}, with
Gate operations can only be executed when the participating qubits are not only adjacent but also co-located within a designated gate zone along the 1D trap. (2) Different operations (e.g., gates, intra-trap movements, inter-trap movements) have significantly distinct latencies \cite{03_03_ion_operation_time}. 
% (3) Inter-trap movements must be performed globally and cannot be performed with intra-trap movements simultaneously. 
(3) Inter-trap ion movement is globally synchronized \cite{02_25_grid_ion_hardware}: all junctions must perform the same type of movement in the same direction, which cannot overlap with intra-trap operations.

While these execution rules can be framed as hardware constraints, we view them instead as architectural features that open up new opportunities for optimization. In fact, the transport behavior of QCCD systems—particularly the globally synchronized inter-trap movement and the performance benefits of grouped intra-trap shifts—closely mirrors the Single Instruction Multiple Data (SIMD) paradigm in classical computing~\cite{classical_simd}. 
%We observe that these system-level constraints give rise to execution behaviors that \emph{closely resemble} the Single Instruction Multiple Data (SIMD) paradigm in classical computing~\cite{classical_simd}.  
At the inter-trap level, globally synchronized movement patterns mimic SIMD instructions broadcasting a uniform command to multiple datapaths. Within a single trap, even if the hardware allows flexible individual ion shifts, it can be beneficial to group ion shift operations together (e.g., moving ions in consecutive positions toward an empty slot) due to their shorter latency than intra-trap ion swaps. This grouping can yield better performance by reducing routing depth and supporting efficient pipelining.
% grouping shifts yields better performance and routing efficiency by enabling position reuse and reducing transport overhead. Together, t
These behaviors highlight the need for architectural abstractions and compilation optimizations that are explicitly aligned with the SIMD-style execution on TI systems.
% \textcolor{red}{(Jens: the phrase ``must be performed globally'' is hard to understand.)}
% Without loss of generality, we illustrate the architectural features of such modular TI systems with the quantum processor developed by Quantinuum --- a leading company in TI quantum hardware, whose implementation reflects the broader direction of the TI community \cite{malinowski2023wire, 02_26_modular_ion_trap, 03_02_qccd_old_version} and exemplifies many of the capabilities and constraints present in TI systems~\cite{03_02_new_ion_hardware, 02_25_grid_ion_hardware}. These  include: (1) Positions in 1D traps are divided into gates zones and auxiliary zones, with gates allowed only in the gate zones. (2) In each 1D trap, multiple shift or swap operations can be performed concurrently as long as their sources/destinations do not conflict, with shift and swap taking different durations of time. (3) Through 2D junctions, ions can be moved globally  by either shift or swap operations in a specified direction. However, the inter-trap movement through 2D junctions conflict with intra-trap movement -- they cannot be performed simultaneously.

%1D traps are typically divided into zones that either support gate operations or serve as auxiliary holding areas. Two-qubit gates are only allowed in gate zones, requiring neighboring ions to be transported into and out of those zones before and after the gate execution. Junctions connecting multiple 1D traps support inter-trap transport via shift or swap operations, but impose global constraints on when and how those operations can be executed.

% \textcolor{red}{SIMD: individual to group, flexibility to optimization; new constraint, also require SIMD}

% We identify that 
% Existing compilers fail to capture many architectural nuances of emerging TI systems, as they are fundamentally based on a Single Instruction Single Data (SISD) paradigm.
However, existing TI quantum compilers~\cite{02_28_shaper, 03_02_qccdsim} are still fundamentally based on a Single Instruction Single Data (SISD) \cite{SISD} execution model, which lacks the ability to express or leverage the SIMD-style behaviors inherent to QCCD architectures. For example, while these SISD compilers may occasionally produce grouped ion shift patterns, they do not actively search for or exploit them. Even if a SIMD-style grouping can be applied as a post-processing step after initial scheduling, many opportunities for grouped ion movements have already been lost due to early gate-level constraints and suboptimal routing decision. As a result, ion movement instructions often become fragmented and uncoordinated, leading to underutilized transport bandwidth.
% \textcolor{red}{(Jens: replace ``identify'' with ``observe''. Or, perhaps drop ``We [,,,] that'' entirely.)}
% In contrast, these TI systems exhibit execution behavior that inherently favors Single Instruction Multiple Data (SIMD). 
% \textcolor{red}{(Jens: I think the ``In contrast'' is a poor wording here because the first sentence of the paragraph has the subject ``existing compilers'' while the second sentence has the subject ``these TI systems'', which is different.)}
% On one hand, it is beneficial to group intra-trap shift operations that can be conducted concurrently, as their latency is distinct from intra-trap swap. 
% \textcolor{red}{(Jens: could we be more specific than ``distinct from''?  Something like ``much longer'' or ``much shorter'' would more specific.)}
% While SISD compilers may occasionally produce such patterns, they do not actively search for or exploit them, resulting in missed optimization opportunities. On the other hand, inter-trap movements are constrained to be global: all ions must move in the same direction using the same operation type. This constraint naturally requires SIMD-style execution, where a single instruction governs the movement of multiple ions.

% We identify that existing compilers fail to capture many architectural nuances of TI machines, as they employ Single Instruction Single Data (SISD) instructions. However, these emerging modular TI systems exhibit execution behavior that is inherently Single Instruction Multiple Data (SIMD) in nature. On one hand, it is advantageous to group intra-trap ion shifts in the same direction and conduct them concurrently, as they share a same duration that differs from intra-trap swaps. While SISD compilers may occasionally produce such grouped patterns, they do not actively seek them out, missing potential optimization opportunities. On the other hand, the constraint of inter-trap ion movements being global requires all ions to be moved collectively in a same direction, this means each inter-trap instruction should indicate the movements of multiple ions.

% Traditional quantum hardware abstractions—typically consisting of an instruction set architecture (ISA) and a qubit coupling graph—fail to capture many architectural nuances of trapped-ion (TI) machines. In particular, many emerging TI systems, especially those built on QCCD models, exhibit execution behavior that is inherently Single Instruction Multiple Data (SIMD) in nature. Without an abstraction that captures this, current compilation pipelines either underutilize available hardware parallelism or introduce significant control overhead.

% \textcolor{blue}{In this work, we address two key challenges in compiler design for modular TI systems built on QCCD architectures: (1) how to develop a hardware-compatible abstraction that captures the system’s transport behavior, gate zone constraints, and scheduling exclusivity, and (2) how to design compilation passes that effectively leverage the resulting design space for optimized performance.}

% In this work, we investigate how to optimize quantum program compilation for a modular TI system.
To exploit the unique features of such systems, we propose a novel abstraction that reflects their SIMD-style ion movement patterns. 
% \textcolor{red}{(Jens: I think we can drop ``framework''.)} 
First, we abstract a set of SIMD-style instructions that models coordinated ion movements both within and across ion trap segments. These include a class of segmented intra-trap shift SIMD (S3) instructions, with each instruction dictating grouped intra-trap ion shifts in a specified direction, and a class of global junction transportation SIMD (JT-SIMD) instructions, with each instruction dictating a global inter-trap operation on selected ions along a specified direction. Second, we inroduce a SIMD-enriched architectural graph abstraction. It augments the traditional coupling graph by capturing TI execution constraints such as the conflict between intra-trap and inter-trap movements, position-awareness, and thermally constrained gate zones.

\begin{figure*}[t!]
        \centering
        \includegraphics[width=\linewidth, trim=0in 0in 0.2in 0in, clip]{fig/intro.pdf}
        
        \caption{Overall Flow of Our Compiler}
        \label{fig:intro_flow}
\end{figure*}

Despite the advantages offered by these abstractions, compile-time optimization under this framework remains highly challenging due to the expansive and constrained design space they introduce. First, within the S3 class, there are numerous candidate S3 instructions, each specifying a set of ions to shift in a particular direction. These instructions can conflict by targeting overlapping destinations, requiring the compiler to carefully select a subset of non-conflicting S3 instructions to maximize execution efficiency. Second, JT-SIMD instructions not only conflict with each other but also with intra-trap operations. Consequently, the compiler must make critical scheduling decisions regarding when to switch between intra-trap and inter-trap execution, and which JT-SIMD instruction to apply when in inter-trap mode.

% However, compilation optimization with these novel abstractions is highly challenging due to the vast design space they create. First, within the S3 class, there can be numerous options for selecting the moved ions and directions. These S3 can conflict with each other by contending for the same destination. Hence we need to identify a set of non-conflicted S3 instructions that maximizes the efficiency of program execution. Second, due to the conflict between different JT-SIMD instructions and their conflict with S3 instructions, at each time only one of the JT-SIMD instructions or a set of S3 instructions can be executed. Hence the choice among different JT-SIMD instructions and the switch between S3 and JT-SIMD instructions is critical to the program execution.

%This paper is based on the combination of the latest hardware technologies of Quantinuum, a leading competitor in TI systems. In their latest H2 processor \cite{03_02_new_ion_hardware}, \textbf{1D ion traps} have been realized with fast and high-fidelity ion transportation within each trap, including ion shift (i.e., moving an ion to an empty location) and ion swap (i.e., switching the locations of two neighboring ions). Recently, Quantinuum has also proposed a novel \textbf{2D junction} \cite{02_25_grid_ion_hardware} to connect 1D ion traps into a 2D grid, thereby overcoming the scalability limitations of 1D ion traps, including the increasing control and calibration overhead as the number of ion increases \cite{malinowski2023wire}[?][?], with a modular architecture.

% As shown in Fig.~\ref{fig:intro_hardware}, in Quantinuum's architecture~\cite{}, each 1D trap is divided into interleaved gate zones (depicted in yellow) and auxiliary zones (depicted in gray), with single-qubit (1Q) gates supported in gate zones and two-qubit (2Q) gates supported between qubits in gate zones and their neighbors (i.e., moving the neighbor into the gate zone, implementing the gate and moving back). Each junction can connect four 1D traps with its four legs, with transportation allowed between the ion locations on the edge of the connected 1D traps, including ion shifts and ion swaps. 


% We base our work on the combination of latest hardware technologies of TI systems. For 1D traps, we adopt the trap design of the H2 hardware of Quantinuum \cite{03_02_new_ion_hardware}. It divides a trap into interleaved gate zones and auxiliary zones, with fast and high-fidelity supported for qubits in the gate zones,  fast and high-fidelity ion transportation, including ion shift and ion swap, supported within the whole trap. For 2D junctions, we adopt the four-leg junction that has been recently realized by Quantinuum \cite{02_25_grid_ion_hardware}. It can connect four 1D traps with its four legs, allowing ion transportation, including ion shift and ion swap, between the edge qubits of the four traps. This combination enables a modular grid structure, facilitating the scalability of future TI processors.



% However, this emerging architecture brings new challenges for compilation, which cannot be resolved by existing compilers. First, this architecture comes with its own hardware constraints. Among 1D traps, operations can only be performed globally across all junctions. That is, while each ion can choose to \emph{stay-or-move} during a global transportation, inter-trap transportation is not allowed to be conducted concurrently with intra-trap transportation (Fig.~\ref{fig:intro_hardware}(a)). Furthermore, all moved ions must be transported by the same type of operation (Fig.~\ref{fig:intro_hardware}(b)), either \emph{shift-or-swap}, along the same direction, e.g., all from the left leg to the bottom leg (Fig.~\ref{fig:intro_hardware}(c)). 
% This constraint is unique for the latest four-leg junction technology, which requires additional awareness by the compilation optimization.

% Second, in each 1D trap, gate operations can only be conducted in the gate zones, while the auxiliary zones can only be used to hold ions. This restricts the computation resource and can cause severe contention for gates zones if not carefully optimized. Existing TI compilers [?] routes ions by identifying a suitable path, lacking coordination between different ions and different types of transportation. This can easily lead to congestion, due to both the conflicts between different paths and the contention for the limited gate zones. 

% Third, none of existing frameworks can fully utilize the flexibility enabled by the latest hardware: traditional TI compilers [?][?] do not support native ion swap operation. In a 1D trap, they utilize SWAP gates to swap qubit data, resulting in lower operation fidelity, as the fidelity of SWAP gates is much lower than ion transportation. Among 1D traps, each native in-place ion swap operation would be translated to multiple ion shifts, incurring unnecessary overhead. Compilers for other gate-based platforms are also suboptimal: compilers for superconducting platforms [?][?] cannot leverage the ability of concurrently shifting multiple ions in TI systems, while compilers for neutral atom platforms [?][?] are not aware of the 1D geometry of ion traps.

% Third, the performance distinction between different operations introduces heterogeneity to the computing system. Specifically, ion transportation is slower than gate operations, with inter-trap transportation being slower than intra-trap transportation, and ion swap being slower than ion shift. In order to achieve computation efficiency, it is essential to carefully interleave different operations to minimize their wait time. However, this multi-hierarchy performance cannot be captured by a simple abstraction such as the circuit depth in traditional gate-based compilers. Rather, it requires a fined-grained coordination taking fidelity and latency of different operations into account.\todo{may add quantitative time information at the order-of-magnitude level}



% \begin{figure*}[t!]
%         \centering
%         \includegraphics[width=0.96\linewidth]{fig/intro_flow2.pdf}
        
%         \caption{Overall flow of our compiler.}
%         \label{fig:intro_flow}
% \end{figure*}


% To overcome these challenges, we identify three aspects that require novel techniques. (1) A new abstraction of the hardware structure is required to capture the features and constraints of native operations of the latest TI hardware.  (2) A congestion-aware router is necessary to enable efficient transportation while being aware of the difference between gates zones and auxiliary zones.(3) A latency-aware scheduler is needed to compactly interleave different operations, so that the wait time of distinct operations can be minimized, thereby leading to an efficient compilation.

% We introduce a SIMD Aggregation Pass to systematically merge scalar ion movements into wider SIMD-style instructions. The pass starts by identifying qubits involved in upcoming gates and their nearby empty sites. Guided by a constraint-aware heuristic cost function, it generates candidate shifts to bring qubits closer to each other and to gate zones. To handle contention for empty space, the pass branches the shift strategy whenever multiple ions target the same site. Due to the 1D trap structure, the total number of branches is bounded by $2\times$ the number of conflicts. After all candidate ions are processed, the branch with the lowest heuristic cost is selected. Finally, shift operations in the same direction are aggregated into S3 instructions to enable efficient SIMD-style intra-trap execution.

To this end, we propose a novel TI compiler based on the SIMD-style instructions and enriched architectural abstractions, which consists of two key compilation passes, as shown in Figure~\ref{fig:intro_flow}. 
% \textcolor{red}{(Jens: the text should refer to Figure~\ref{fig:intro_flow}.)} 
First, we introduce a \textbf{SIMD Aggregation Pass} (yellow box in Figure~\ref{fig:intro_flow}) to systematically aggregate scalar ion movement operations into wider SIMD-style instructions. This pass employs a zone-aware cost function to evaluate the figure of merit of each individual operation and the overall movement strategy formed by their aggregation. To find a more global optimum than a greedy operation search, it performs a branching algorithm that splits a potential movement strategy into two alternative plans whenever multiple ions target the same empty site. Due to the linear structure of 1D ion traps, the total number of branches is bounded by $2\times$ the number of contended sites. After all candidate ions are processed, the branch with the lowest cost is selected. Then, shift operations in the same direction in this branch will be aggregated into S3 instructions to enable efficient SIMD-style intra-trap execution.

% precise but not high-level enough
% This pass begins by identifying qubits involved in upcoming gates and their nearby empty locations. Guided by a carefully designed zone-aware heuristic cost function, it generates candidate shift operations to bring qubits closer to each other and closer to gates zones. \textcolor{red}{(Jens: I suggest that we drop ``heuristic''.  If ``heuristic'' is important to you, then write one sentence that explains what it means and then drop ``heuristic'' whenever you later talk about the cost function.)} Instead of employing a simple greedy approach, our pass resolves empty space contention by branching the shift plan: when multiple ions target the same empty site, the shift plan is split into two alternative branches. Owing to the linear structure of 1D ion traps, the total number of branches is bounded by $2\times$ the number of contended sites. After all candidate ions are processed, the branch with the lowest heuristic cost is selected.  Finally, shift operations in the same direction are aggregated into S3 instructions to enable efficient SIMD-style intra-trap execution.

% Once all candidate ions have been processed, the pass compares the overall heuristic costs of each branch to select the most efficient shift configuration. Finally, individual shift operations in the same direction are aggregated into a set of S3 instructions, enabling efficient SIMD-style intra-trap execution.


% It identifies ions involved in upcoming gates along with their nearby empty locations, then finds candidate individual shift operations with the guidance of a constraint-aware heuristic cost function. Instead of forming a shift strategy by a greedy search, it splits a candidate shift strategy into two branches whenever empty space contention occurs, with the number of total branches bounded by $2\times$ the number of contended empty spaces due to the linear structure of 1D traps. After depleting all qubits that intend to shift, the overall heuristic costs of these branches would be compared to determine the best shift strategy. Finally, shifts in the same direction would be grouped into multiple S3 instructions.

Second, we employ a \textbf{SIMD Scheduling Pass} (green box in Figure~\ref{fig:intro_flow}) to select and schedule SIMD instructions under hardware constraints. This pass adopts a scheduling policy that prioritizes low-latency intra-trap movements, deferring high-latency inter-trap operations until they become urgent or sufficient gain has accumulated. At each timestep, it performs a hierarchical decision process: (i) evaluating all candidate JT-SIMD instructions with the heuristic cost function and then (ii) comparing the best JT-SIMD option against the cost of continuing with intra-trap execution. The compiler switches to JT-SIMD only when its benefit substantially outweighs that of intra-trap execution, thus naturally encouraging the grouping of more inter-trap
movements into a single JT-SIMD instruction. To handle the distinct latencies of different operations, the pass incorporates a time-sliced synchronization mechanism that maintains a fine-grained view of the system’s execution state. This enables more precise scheduling decisions and reduces qubit idleness by issuing new instructions as soon as hardware resources become available.

% Second, we employ a \textbf{SIMD Scheduling Pass} to select and schedules SIMD instructions under hardware constraints. The pass adopts a selection policy that favors intra-trap movements for their lower latency, deferring high-latency inter-trap operations until sufficient parallelism can be exploited. At each timestep, it evaluates all candidate JT-SIMD instructions with the heuristic cost function and compares the best JT-SIMD option with the cost of continuing intra-trap S3 execution. The compiler proceeds with JT-SIMD only if its benefit clearly outweighs that of S3, with this deferral of switching naturally encourages the grouping of more inter-trap movements into a single JT-SIMD instruction. To handle the distinct latencies of various operations, the pass incorporates a time-sliced synchronization mechanism that maintains a fine-grained view of the system’s execution state. This enables more precise scheduling decisions and reduces qubit idleness by initiating new instructions as soon as hardware resources become available.

% Second, we employ a \textbf{SIMD Scheduling Pass} to select and schedule SIMD instructions under hardware constraints. It determines which SIMD instructions to prioritize at each moment in time by a hierarchical decision process: it selects the optimal JT-SIMD instruction by comparing the heuristic cost of candidate JT-SIMD instructions, prioritizing intra-trap movement and switching to JT-SIMD only when its cost is significantly lower. This delays the more latent inter-trap movements until necessary, which naturally group more inter-trap movements in the JT-SIMD instruction. The distinct latency of different instructions is then handled by a time-sliced SIMD synchronization mechanism, which enhances scheduling precision and minimizes qubit idle time by tracking real-time execution information.


% \textbf{SIMD Scheduling Pass} selects and schedules SIMD instructions under hardware constraints, deciding which movements to perform at each timestep based on routing urgency, control resource availability, and gate zone pressure. Together, these passes align the software execution schedule with the physical movement capabilities of QCCD hardware, enabling scalable and performance-aware compilation beyond conventional scalar instruction strategies.



% Once SIMD instructions are formed, they must be scheduled under hardware constraints. A naive scheduling may introduce excessive junction contention, control overhead, or thermal violation. We therefore perform cost-aware planning across time steps.

% At a high level, many SIMD instructions---whether intra-trap S3 or inter-trap JT-SIMD---enable ion movement that brings qubits closer together for upcoming two-qubit gates. However, only a subset of these instructions can be executed at any given time due to architectural constraints. The goal of this scheduling pass is to determine \emph{which} SIMD instructions to prioritize at each moment in time, so as to minimize total routing cost while maintaining gate readiness.

% To execute aggregated SIMD instructions efficiently, the compiler
% must schedule them under hardware constraints such as control ex-
% clusivity and thermal limitations. This section presents a two-stage
% strategy: first, a hierarchical decision process selects the optimal
% JT SIMD instruction class and determines whether to prioritize
% intra- or inter-trap operations; second, a time-sliced SIMD synchro-
% nization mechanism coordinates operations at the sub-cycle level,
% improving latency handling and overall throughput. Together, these
% scheduling techniques maximize gate readiness while minimizing
% system contention and routing delay.


% To this end, we propose an abstraction that we call the \textbf{switchable position graph}. The vertices in this graph stand for possible ion locations, where each location can be occupied by an ion or be empty; the edges represent the neighborhood relations between the locations. To comply with the hardware constraints, edges in the graph are not always active, but switch between several patterns: (1) all intra-trap edges are active while all inter-trap edges are inactive; (2) all intra-trap edges are inactive while inter-trap edges in a certain direction of all junctions are active. Compared to prior work, it changes the description of system status from the view of ions to the view of possible locations. This not only allows an easy integration with existing gate-based compilers, but also lays a foundation for the subsequent  optimizations.


% We then propose a \textbf{step-by-step router} with a carefully designed cost function to further optimize the transportation trajectory of each ion. In contrast to previous compilers which first search for end-to-end routing paths and then detect congestion, it implements a more fine-grained search with each transportation only taking a single step from a location to its neighborhood, thereby naturally preventing congestion and allowing more flexibility for routing. The heuristic function enables 2Q gates by minimizing both the distance of between corresponding ions and between the ions and gate zones, taking all gates in the near future into account in a weighted manner. It further employs a priority among different 2Q gates to prevent contention for the limited gate zones.

% Lastly, we propose a \textbf{simulator-based just-in-time (JIT) scheduler} to coordinate the routing of different types of ion transportation. Specifically, it schedules one round of inter-trap transportation after certain rounds of intra-trap transportation, with the number rounds adjusted by an auto-tuned parameter. In each intra-trap round, it schedules multiple concurrent ion shift and ion swap operations, enabling grouped ion shift by carefully managing the empty locations and searching for ion shift before ion swap. The scheduler is JIT in the sense that, after the processing of each instruction by the discrete event simulator, it updates the circuit status, empty locations and the remaining time of incomplete instructions, so that it only needs to hold information about the current status. This updating mechanism makes the scheduling more compact by taking the latency discrepancy between different operations into account, enabling discovery of more optimization opportunities.



Our contributions in this paper can be summarized as below.
\begin{itemize}
    \item We propose a novel SIMD abstraction that captures the features of modular TI architectures by a set of SIMD-style instructions and SIMD-enriched architectural graph abstraction, enabling optimized compilation tailored to TI systems.
    \item We introduce a SIMD aggregation pass to systematically aggregates scalar ion movement operations into wider SIMD instructions, which identifies the most effective SIMD instructions by a branching strategy with a carefully designed heuristic cost function.
    \item We employ a SIMD scheduling pass to optimize the scheduling of SIMD instructions under hardware constraints, which enhances execution efficiency by a strategic selection and switching between different SIMD instructions, coordinated by a time-sliced synchronization.
    
    \item Through a comprehensive evaluation, we demonstrate that our compiler, incorporating these novel techniques, improves execution time by a factor of 2.90x and significantly enhances fidelity by several orders of magnitude.
    \textcolor{red}{(Jens: mention that we have both NISQ and FTQC benchmarks.)}
\end{itemize}




==> 03_background_and_related_work.tex <==
\section{Background and Related Work}\label{sect:background}

This section provides essential background information on trapped ion hardware capabilities and architectures. We first introduce the scalable charge-coupled device (QCCD)  architecture, and then present the fidelity and duration of each operation, including gate operations, measurements, and ion movement.

\subsection{Trapped Ion Architectures}
Trapped-ion quantum computing stores quantum information in the internal state of electrically charged ions. It is one of the leading approaches to realizing high-fidelity quantum operations. To overcome the scaling difficulties of a single trap, quantum QCCD architecture was proposed to utilize multiple traps by transporting ions between different traps using dynamic electric fields \cite{QCCD_1,QCCD_2,03_02_new_ion_hardware}, with each trap containing a small number of ions. 


\noindent\textbf{1D Single Traps} Within each ion trap, ions are arranged in a 1D linear chain. Existing 1D traps either feature full connectivity between ions directly or achieves full connectivity by allowing ion transportation within the trap. The latter approach mitigates the control and calibration overhead as it consists of less gate zones that are interleaved with auxiliary zones
% \textcolor{red}{(Jens: the phrase ``less and more'' is confusing)} 
in each trap [?][?]. Yet it still suffers from scalability challenges as the transportation overhead increases with the length of ion traps. 

In the latest hardware technology including Quantinuum's H2 processor, gate zones in a trap are interleaved with auxiliary zones where ions can only be held. High-fidelity 1Q gates, 2Q gates and measurements can be conducted in the gate zones. In the absence of 2Q gates, each gate zone or auxiliary zone is occupied by a single ion at most. When a 2Q gate is needed, two ions are moved to a gate zone, conducting a 2Q gate through a laser pulse on both of them, and moving one of them away from the gate zone, as shown in Fig.~\ref{fig:background_2Q}. Ion transportation can be conducted in two ways: ion shift (or shuttling) and ion swap \cite{02_25_ion_CCD, 03_02_new_ion_hardware}. The former moves a ion to along empty locations in the trap, while the latter exchanges the locations of two neighboring ions. 
% To allow enough space for ion shift, the number of ions in each trap is usually restricted below its maximum capacity, usually restricted to ?? to ?? ions \cite{?}.

% \noindent\textbf{1D Single Traps} Within each trap, ions are arranged in a 1D linear chain, with reliable single-qubit (1Q) gates and two-qubit (2Q) gates allowed with full connectivity, as well as qubit measurements. These operations can be conducted only in specific locations in the trap, called a \emph{computation zone}, while other locations can only hold the ions without operations. These ions can be moved (or transported) in two ways: ion shift (or shuttling) and ion swap \cite{02_25_ion_CCD, 03_02_new_ion_hardware}. Ion shift moves a ion to along empty locations in the trap, while ion swap exchanges the positions of two neighboring ions. To allow enough space for ion shift, the number of ions in each trap is usually restricted below its maximum capacity, usually restricted to ?? to ?? ions \cite{?}.

\begin{figure}[h!]
        \centering
        \includegraphics[width=\linewidth]{fig/background_2Q.pdf}
        
        \caption{2Q gate implementation in a 1D trap.}
        \label{fig:background_2Q}
\end{figure}

\noindent\textbf{2D Junctions} In the QCCD architecture, the scalability challenges of 1D traps are overcome by connecting different traps by junctions, which allow ions to be transported between different traps. Specifically, ions on the edge of a trap can be transported on the edge location of another trap. Previous hardware technology only allows ions to be shifted to an empty edge location of another trap through the so-called Y-junction \cite{02_28_shaper, 03_02_qccdsim}. Recently, hardware advancements have also enabled on-site swap between different edge ions \cite{02_25_grid_ion_hardware}. This new type of junction consists of four legs, forming a crossing shape, thus enabling a 2D grid structure of connected traps. 

\begin{figure}[h!]
        \centering
        \includegraphics[width=\linewidth]{fig/background_inter.pdf}
        
        \caption{Inter-trap transportation through a junction.}
        \label{fig:background_inter}
\end{figure}

However, these movements come with constraints. First, at each round, we need to choose a single type of inter-trap operation: either shift or swap. Except specified fixed ions, all the ions would be transported globally. Second, at each round, the inter-trap shift or swap operation can only be conducted along a single direction. That means, all unfixed edge ions would be transported, for example, from the left leg to the bottom leg of the junctions. 

% The quantum charge-coupled device (QCCD) architecture is a scalable method for trapped-ion quantum computation \cite{QCCD_1,QCCD_2,03_02_new_ion_hardware}. To address the limitation in qubit number of a single trapping trap, it supports multiple trapping traps and allows operations to always be performed with a small number of ions, thereby facilitating low-crosstalk addressing and maintaining high fidelity \cite{QCCD_3}.



\subsection{Operation Fidelity and Duration}
% On TI platforms, qubit information is stored in the internal states of ions. These qubits can conduct fast single-qubit (1Q) and two-qubit (2Q) gates with a high fidelity, by stimulated Raman processes described in \cite{02_25_ion_CCD}. 
In this paper, we adopt the fidelity and duration of TI-platform gates from the latest experimental and architectural papers \cite{03_02_new_ion_hardware,02_25_grid_ion_hardware,02_25_ion_CCD}, as listed in Table~\ref{tab:hardware_data_table}. 

\noindent\textbf{Gates and Measurements} In general, measurement operations on a TI platform are more expensive than gates, while 2Q gates are more expensive than 1Q gates. Specifically, the fidelity of 1Q gates is $99.9975\%$ \cite{03_02_new_ion_hardware},
% (infidelity  $2.5\times10^{-5}$ \cite{03_02_new_ion_hardware}) 
while the fidelity of 2Q gates is $99.82\%$ \cite{03_02_new_ion_hardware}. 
% (infidelity $1.8\times10^{-3}$ \cite{03_02_new_ion_hardware}). 
Typically, each 1Q gate takes $5\mu s$ \cite{02_25_ion_CCD} while each 2Q gate takes $25\mu s$ \cite{02_25_ion_CCD}. Moreover, 1Q measurement has a fidelity of $99.84\%$ \cite{03_02_new_ion_hardware} and a duration of $120\mu s$ \cite{02_25_ion_CCD}.

\noindent\textbf{Ion Movements} For movement fidelity, both intra-trap and inter-trap movement, including qubit swap and qubit shift, have a similar fidelity of $99.978\%$ \cite{03_02_new_ion_hardware}.
% For movement duration, however, qubit swap is slower than qubit shift, with inter-trap movements being slower than intra-trap movements.
The movement durations are different, however, with qubit swap being slower than qubit shift.
Specifically, the duration of intra-trap qubit shift is $58 \mu s$ \cite{02_25_ion_CCD}, the duration of intra-trap shift is $200 \mu s$ \cite{02_25_grid_ion_hardware}, the duration of inter-trap qubit swap is $200 \mu s$ \cite{02_25_ion_CCD} and that of inter-trap qubit swap is $500 \mu s$ \cite{02_25_grid_ion_hardware}.
% \textcolor{red}{(Jens: something is inconsistent here; specifically, the text says that inter-trap movements are slower than intra-trap movements, but the numbers say that both can be $200 \mu s$, in some cases.)}

\noindent\textbf{2Q Gate on Adjacent Ions} As shown in Fig.~\ref{fig:background_2Q}, a 2Q gate can be performed on ions with adjacent positions as long as one of them is in a gate zone. This is achieved by shifting the other qubit to the same gate zone, applying a laser pulse and shifting it back to the original position. This leads to an overall fidelity of 99.776\% and an overall latency of $141\mu s$ when the shift is intra-trap, or an overall fidelity of 99.732\% and an overall latency of $425\mu s$ if the shift is inter-trap. \textcolor{red}{(Jens: this would be a missed opportunity to show a difference from the usual 2-qubit-gates-on-neighbors-only.)}

\begin{table}[h]
\caption{Fidelity and latencies of TI operations}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{|l|l|l|}
\hline
operation              & fidelity                               & duration ($\mu s$)      \\ \hline
1Q gate                & 99.9975\% \cite{03_02_new_ion_hardware}                                                                           & 5 \cite{02_25_ion_CCD}              \\ \hline
2Q gate                & 99.82\% \cite{03_02_new_ion_hardware}  & 25 \cite{02_25_ion_CCD}             \\ \hline
measurement            & 99.84\% \cite{03_02_new_ion_hardware}  & 120 \cite{02_25_ion_CCD}            \\ \hline
intra-trap qubit shift & 99.978\% \cite{03_02_new_ion_hardware} & 58 \cite{02_25_ion_CCD}             \\ \hline
inter-trap qubit shift & 99.956\% \cite{03_02_new_ion_hardware} & 200 \cite{02_25_grid_ion_hardware} \\ \hline
intra-trap qubit swap  & 99.978\% \cite{03_02_new_ion_hardware} & 200 \cite{02_25_ion_CCD}            \\ \hline
inter-trap qubit swap  & 99.912\% \cite{03_02_new_ion_hardware} & 500 \cite{02_25_grid_ion_hardware} \\ \hline
\end{tabular}
}
\label{tab:hardware_data_table}
\end{table}

\noindent\textbf{Gate-based vs Ion-based Swap}
There are two standard ways of performing ion reconfiguration within each trap: gate-based swapping and physical ion swapping. The former approach utilizes SWAP gates to swap the quantum states of the desired ions. Each SWAP gate can be decomposed to three CNOT gates, resulting in a fidelity of $99.46\%$ and a latency of $75\mu s$. As this fidelity is much lower than the $99.978\%$ fidelity of intra-trap qubit movement, we will adopt the ion-based approach, although it has a longer latency of $200\mu s$.


% \noindent\textbf{Gate operations}
% As one of the original platforms suggested for quan- tum computing more than 25 years ago [1], trapped ion systems have maintained their status as a leading candidate for gate-based quantum processors. Trapped ion qubits have been used to demonstrate the published world records in two-qubit gate fidelity [2, 3], single-qubit gate fidelity [4], and state preparation and measurement error [5]. In conjunction with the all-to-all qubit connec- tivity enabled by ion transport operations [6–8], trapped ion quantum computers have raised quantum computing performance benchmarks such as quantum volume [9] to new heights [10].


% fidelity (new):
% 1-qubit gate fidelity table
% 2-qubit gate
% measurement
% transport fidelity (move/shift and swap) 

% duration 02 25 ion ccd:
% 1-qubit gate
% 2-qubit gate
% measurement
% intra-trap shift 58
% inter-trap shift (02 25 grid ion) 200
% intra-swap (02 25 ion ccd) 200
% inter-swap 500 (02 25 grid ion 200 2.0kHz)

% 1D QCCD
% 2D junction: grid transport



==> 04_motivation.tex <==
\section{Motivation}\label{sect:motivation}

% \begin{figure*}[t!]
%         \centering
%         \includegraphics[width=\linewidth]{fig/motivation_JIT.pdf}
        
%         \caption{Motivating example of our compiler.
%         % \textcolor{red}{(Jens: can each $C(X)$ gate be shown with a filled circle on the control qubit please? This way we know that the control is on 1, rather than on 0.  I know the operation of the gate is irrelevant to the example but I see no need to change the usual diagram symbols.)}
%         \textcolor{red}{(Jens: The listing of gate blocks is missing SG. 
%  Also, in (c4), why does one of the TG gates in the middle column start ``a little late''? It looks odd and comes with no explanation in the text.  I think (c4) could have the labels Q1--Q5, like (b5).  Also, no need to show the inter-trap shift in this figure.)}
%         }
%         \label{fig:motivation}
% \end{figure*}

\begin{figure*}[t!]
        \centering
        \includegraphics[width=\linewidth]{fig/motivation.pdf}
        
        \caption{Motivating example of our compiler.  
        % \textcolor{red}{In (c4), we lost a qubit! Find it and bring it back :-).  I think (c4) could have the labels Q1--Q5, like (b5).}
        }
        \label{fig:motivation}
\end{figure*}

We propose a novel compiler to overcome the challenges brought by the new native operations, the distinction between different operations and the hardware constraints in the emerging TI architecture. This section introduces the optimizations in our compiler with motivating examples.

% Fig.~\ref{fig:motivation} demonstrates an example of compiling the circuit in Fig.~\ref{fig:motivation}(?) onto two? 1D ion traps with an initial qubit mapping shown in Fig.~\ref{fig:motivation}(?). \textcolor{red}{(Jens: where is the initial qubit mapping shown?  If it is the diagram just below the circuit in Fig.~\ref{fig:motivation}, then say more about what it shows.)} The 1D ion traps are connected by a ? junction. 
% For simplicity, we do not distinguish gate zones and auxiliary zones with each 1D trap, assuming that all locations are gate zones.

\subsection{Awareness of Latency-discrepancy}
When applied to TI systems, existing gate-based compilers has a drawback of overlooking the disparity between latencies of different operations. This can lead to a suboptimal scheduling, as demonstrated in Fig.~\ref{fig:motivation}(b1)--(b5).

In Fig.~\ref{fig:motivation}, the TI systems intends to implement the circuit in Fig.~\ref{fig:motivation}(a1) with an initial layout in Fig.~\ref{fig:motivation}(a2). Being unaware of latency disparity, existing gate-based compilers [?] (\todo{cite}) would schedule the operations in the following steps, with the layout after each step shown in Fig.~\ref{fig:motivation}(b1)(b2)(b3) respectively. \textbf{Step 1:} As shown in Fig.~\ref{fig:motivation}(b1), the 1Q gate is conducted on Q4. 
% \textcolor{red}{(Jens: this isn't really shown in (b1); I think you can drop ``As shown in'' and rephrase a little bit.)} 
Concurrently, Q1 and Q3 are brought adjacent by swapping Q1 with Q2. \textbf{Step 2:} As shown in Fig.~\ref{fig:motivation}(b2), the 2Q gate between Q1 and Q3 is conducted. Meanwhile, Q4 is shifted up to become adjacent to Q3.
\textbf{Step 4:} As shown in Fig.~\ref{fig:motivation}(b3), the 2Q gate between Q3 and Q4 is conducted. Concurrently, Q5 is shifted up to get closer to Q3. \textbf{Step 3:} As shown in Fig.~\ref{fig:motivation}(b4), Q5 is brought adjacent to Q3 by swapping with Q4. Then, the 2Q gate between Q3 and Q5 is conducted. 
% \textcolor{red}{(Jens: the text in this paragraph matches (b1)-(b3) nicely, while it matches (b4) less well.  The problem is that the three steps don't line up with the columns in the schedule.  One idea is to move ``Then, the 2Q gate between Q1 and Q3 can be conducted'' from the text about Step 1 to the text about Step 2.  Another idea is to add text about that column 3 in (b4) contains both two TGs from Step 2 and an SH from Step 3.)}

This scheduling is represented by Fig.~\ref{fig:motivation}(b5), with each row representing a qubit and each block representing an operation. For example, two `SW' blocks in the first and second row stand for a swap between Q1 and Q2, while two `TG' blocks in the first and third row of the second column stand for a 2Q gate between Q1 and Q3. If we give each block a length that is proportional to the latency of the operation, then we get \ref{fig:motivation}(b6), with an identification that the two shift operations can actually be conducted simultaneously.
% According to the latency of each operation, the scheduling should be translated to that in \ref{fig:motivation}(b5), with an identification that the two shift operations can actually be conducted simultaneously. 
This leads to a computation time of $793\mu s$.

% \textcolor{red}{(Add ``Step 1'', etc to Fig.~\ref{fig:motivation}.)} 

% \textcolor{red}{(Jens: this thing about being adjacent is different from the idea of a gate zone.  If you want to keep ``adjacent'', you will have to say that you think of any two adjacent qubits as being in the same gate zone.  But this would be a missed opportunity to show a difference from the usual 2-qubit-gates-on-neighbors-only.)}

% Fig.~\ref{fig:motivation}(a1)-(a5) shows the compilation process with existing gate-based compilers [?]. \textcolor{red}{(Jens: please cite such a compiler.)} \textcolor{red}{(Jens: I think this is the top row of Fig.~\ref{fig:motivation}. About the top left corner of Fig.~\ref{fig:motivation}: add an explanation of why SWAP Q0 Q1 appears twice, and also why G23 appears twice.  Also, add an explanation that G23 stands for a gate that operates on qubits 2 and 3.)} \textbf{Step 1:} It first swaps Q0 and Q1 to bring Q0 closer to Q2. Concurrently, it conducts gate G23 as it identifies that G02 and G23 commute.  \textcolor{red}{Add ``Step 1'', etc to Fig.~\ref{fig:motivation}.)} \textbf{Step 2:} Then, G02 can be conducted since Q0 and Q2 are adjacent now. \textcolor{red}{(Jens: this thing about being adjacent is different from the idea of a gate zone.  If you want to keep ``adjacent'', you will have to say that you think of any two adjacent qubits as being in the same gate zone.  But this would be a missed opportunity to show a difference from the usual 2-qubit-gates-on-neighbors-only.)} Meanwhile, it shifts Q3 to the right and Q1 to the left, in order to enable gate T34 and T15.  \textcolor{red}{(Jens: now the text talks about T34 and T15, which use the letter ``T''; please add an explanation.)} \textcolor{red}{(Jens: I am unable to find a shift of Q1 to the left in Fig.~\ref{fig:motivation}.  Also, what is T15 for?  I don't see anything like a T15 in the circuit diagram.)} \textbf{Step 3:} After that, Q2 is shifted to the right to enable gate G23. \textcolor{red}{(Jens: we have two 2-qubit gates on qubits 2 and 3, but the text refers to both as G23; perhaps do something to distinguish them; could be ``the first G23 gate'' and ``the second G23 gate''.)}

% In this process, the compiler considers the latencies all operations as the same and overlooks the constraint that the left shift of Q1 is an inter-trap operation which conflict with the intra-trap ones. As a result, these steps will be further scheduled as in Fig.~\ref{fig:motivation}(?) in the real program execution, with the number in each block indicating the latency of the operation. This leads to a total latency of 533$\mu s$ for the circuit execution.

% In contrast, our compiler takes the discrepancy of different operations into account and provides a more compact compiled program with a fine-grained scheduling. \textbf{Step 1:} The first step is still swapping Q0 and Q1 to bring Q0 closer to Q2 and concurrently conducting the gate G23. \textbf{Step 2:} However, before conducting the gate G02, we identify that we still have enough time to do something more as the swap of Q0 and Q1 takes a relatively long time. Specifically, we can conduct a grouped transportation of Q2 and Q3, shifting them both to the right. In this way, we can conduct gate G34 and G23 and then shift Q2 back before the end of the swap between Q0 and Q1. \textbf{Step 3:} After that, gate G02 can be conducted as Q2, which has been shifted back, is adjacent to Q0. \textbf{Step 4:} Being aware of the hardware constraints, we schedule a left shift for Q1 after all these intra-trap operations are completed, and then conduct gate G05. This process can be directly translated to a compiled program as shown in Fig.~\ref{fig:motivation}(?), leading to a total latency of 450 $\mu s$ only.

With the awareness of latency disparity, our compiler can produce a better scheduling as shown in \ref{fig:motivation}(c4), which has the following steps. \textbf{Step 1:} As shown in \ref{fig:motivation}(c1), the 1Q gate is conducted on Q4, while Q1 and Q3 are brought adjacent by swapping Q1 with Q2. \textbf{Step 2:} As shown in \ref{fig:motivation}(c2), a grouped shift is conducted on Q4 and Q5 in the up direction to bring them closer to Q3. \textbf{Step 3:} As shown in \ref{fig:motivation}(c3), before the completion of the swap operation, we identify that the 2Q
gate between Q3 and Q4 can also be conducted. We remark that this cannot be identified by previous compilers demonstrated in Fig.~\ref{fig:motivation}(b), despite that the 2Q gate between Q1 and that between Q3 and Q4 are actually commutable. This is because they lack the awareness of grouped ion shift in TI system. Specifically, the shift operation on Q4 and Q5 are scheduled separately in step 2 (Fig.~\ref{fig:motivation}(c2)) and step 3 (Fig.~\ref{fig:motivation}(c3)), which leads the compiler to conduct the 2Q gate between Q1 and Q3 first.
% \textcolor{red}{(Jens: here you are using an optimization that swaps two $C(X)$ gates, namely the one on 13 and the one on 34.  I wonder whether this is entirely fair to the standard compiler.  If you put these glasses on, then the only difference between (b5) and (c4) is this single optimization.  I tend to think that we need a better example.)} 
\textbf{Step 4:} As shown in \ref{fig:motivation}(c4), after the 2Q gate between Q3 and Q4 is completed, we then swap Q4 and Q5 to bring Q4 adjacent to Q3, and conduct the 2Q gate between Q1 and Q3. \textbf{Step 5:} As shown in \ref{fig:motivation}(c5), this is followed by the 2Q gate between Q3 and Q5. 
% \textcolor{red}{(Jens: I suggest that focus this entire paragraph on (c4).  The reason is that earlier text made me understand (b5) really well, which makes (c4) feel like an easy next thing to look at.  You might even remove (c1)-(c3) from Fig.~\ref{fig:motivation}, but if you keep (c1)-(c3), then you need to make them look more like (b1)-(b3), which means that you need to show one more swap in (b1).)} 

The main difference between our scheduling and previous gate-based compilers is that we fill up the time of the swap operation between Q1 and Q2 with the execution of 2Q gate between Q3 and Q4. This is on one hand due to our compiler's ability of identifying grouped ion shift, and on the other hand due to our fine-grained scheduling based on discrete event simulation. Overall, these lead to a shorter computation latency of $525\mu s$. 


\subsection{Awareness of Hardware Constraints}

Another drawback of existing gate-based compilers for TI systems is that they cannot adapt to the unique constraints on ion transportation. For example, their transportation scheduling can be suboptimal in the case shown in Fig.~\ref{fig:motivation}(e1)--(e5), as they are not aware of the constraint that inter-trap transportation cannot be conducted simultaneously with intra-trap transportation. 

In Fig.~\ref{fig:motivation}, the TI system needs to implement a circuit in Fig.~\ref{fig:motivation}(d1) with an initial layout in Fig.~\ref{fig:motivation}(d2). With existing gate-based compilers, operations would be scheduled in the following steps. 
% \begin{enumerate}
%     \item As shown in Fig.~\ref{fig:motivation}(b1), the 2Q gate G23 is conducted as Q2 and Q3 are adjacent. Concurrently, Q1,Q3 and Q2, Q4 are brought closer by an intra-shift on Q1 in the down direction and an inter-shift on Q3 in the down-right direction. Then, the 2Q gate G45 is conducted since Q4 and Q5 are adjacent now.
%     \item As shown in Fig.~\ref{fig:motivation}(b2), Q1 and Q3 are brought further closer by further shifting down Q2 and swapping Q2 and Q3.
%     \item As shown in Fig.~\ref{fig:motivation}(b3), an inter-trap shift on Q1 is conducted to bring Q1 adjacent to Q3, so that the 2Q gate G13 can be conducted now.
% \end{enumerate}
\textbf{Step 1:} As shown in Fig.~\ref{fig:motivation}(e1), the 2Q gate G23 is first conducted as Q2 and Q3 are adjacent. Concurrently, Q1,Q3 and Q4, Q5 are brought closer by an intra-shift on Q1 in the down direction and an inter-shift on Q4 in the down-right direction. Then, the 2Q gate G45 is conducted since Q4 and Q5 are adjacent now. \textbf{Step 2:} As shown in Fig.~\ref{fig:motivation}(e2), Q1 and Q3 are brought further closer by further shifting down Q1 and 
swapping Q2 and Q3. \textbf{Step 3:} As shown in Fig.~\ref{fig:motivation}(e3), an inter-trap shift on Q1 is conducted to bring Q1 adjacent to Q3, so that the 2Q gate G13 can be conducted now.

Taking the conflict between intra-trap and inter-trap transportation into account, this scheduling should be translated to that in Fig.~\ref{fig:motivation}(e5). Note that while the two inter-trap shifts are in the same direction, they are conducted separately, which together lead to a long computation latency of $862\mu s$.

In contrast, our compiler can provide an optimized scheduling by identifying and grouping inter-trap transportation along the same direction. With the same example, our compiler would schedule operations in the following steps, as represented by Fig.~\ref{fig:motivation}(f4). \textbf{Step~1:} As shown in Fig.~\ref{fig:motivation}(f1), the 2Q gate between Q2 and Q3 is first conducted as these qubits are adjacent. Concurrently, Q1 is shifted down for two steps to get closer to Q3. \textbf{Step 2:} As shown in Fig.~\ref{fig:motivation}(f2), Q2 and Q3 are swapped to bring Q3 closer to Q1. \textbf{Step 3:} As shown in Fig.~\ref{fig:motivation}(f3), Q1 and Q4 are shifted in the down-right direction by a global inter-trap transportation to bring them adjacent to Q3 and Q5, so that the two 2Q gates between Q1,Q3 and between Q4,Q5 can be conducted.

The primary optimization in these steps is that our compiler groups the inter-trap shifts on Q1 and Q4 to reduce transportation latency, leading to an overall computation latency of $662\mu s$ only. This grouping is achieved by a careful design of a heuristic function for routing, which collectively schedules a global inter-trap transportation only when the gain is large enough.

% \newpage

==> 05_tech-2.tex <==
\section{SIMD-Aware Compiler Design}\label{sect:aggregation}
\todo{Incorporate Motivation Example 2}
With SIMD-style instructions and enriched architectural abstractions in place, the compiler must translate quantum programs into hardware-efficient execution plans that expose parallelism, respect architectural constraints, and minimize routing cost. Toward this goal, our compiler introduces two key optimization passes tailored to trapped-ion execution: \textbf{SIMD Formation Pass} identifies opportunities to aggregate scalar movement operations into wider SIMD-style instructions, leveraging spatial locality and alignment to form intra-trap S3 and inter-trap JT-SIMD instructions. \textbf{SIMD Scheduling Pass} selects and schedules SIMD instructions under hardware constraints, deciding which movements to perform at each timestep based on routing urgency, control resource availability, and gate zone pressure.
Together, these passes align the software execution schedule with the physical movement capabilities of QCCD hardware, enabling scalable and performance-aware compilation beyond conventional scalar instruction strategies.

\subsection{SIMD Formation Pass: Aggregating Operations into SIMD Instructions}
% The first challenge is to identify opportunities for converting individual ion movement operations into SIMD-style instructions. Rather than issuing ion shifts or transfers one-by-one, we analyze the input quantum program to detect spatially and temporally local patterns of movement that can be bundled together.

% The first challenge is to identify opportunities for converting individual ion movement operations into SIMD instructions. By analyzing the input program, we identify intra- or inter-trap ion movements that can be performed concurrently and aggregate them into SIMD instructions. This is achieved by a staged scheduling that separates the search for intra-trap shift from intra-trap swap, while separating the search for intra-trap movements from inter-trap ones, along with a well-designed heuristic cost function.

The first challenge is to identify opportunities for converting individual ion movement operations into SIMD-style instructions. Rather than issuing ion transportation one-by-one, we analyze the input quantum program to detect spatial and temporal patterns of movement that can be bundled together.

% \noindent \textbf{1. Intra-Trap S3 Aggregation:} For each linear trap segment, we analyze the shift intentions of resident ions over the next few timesteps. If multiple ions within the same segment intend to move in the same direction and do not conflict in source/destination, we group them into a single S3 instruction. This step involves solving a spatial clustering problem with shift-alignment constraints.

% \noindent \textbf{1. Intra-Trap S3 Aggregation:} In the stage of intra-trap movement search, we first analyze the shift intentions of different ions and group them into S3 instructions if multiple ions within the same 1D trap intend to move in the same direction without conflict in source/destination. Specifically, for all qubits involved in 2Q gates over the next few timesteps, we calculate the heuristic cost of its movements in all possible directions and select the ones with the lowest costs. Whenever a shift is selected, we lock the position of its destination, freeing the position of its source so that they can be occupied by subsequent shift. After that, we collect the selected shifts with the same direction within each 1D segment and group them into S3 instructions.

% Then, the intra-trap shift search is followed by a intra-trap swap search that scores all possible swap operations. This separate search for shift and swap enables better S3 aggregation. This is because given the different latencies of shift and swap, once shifts that can be grouped are interrupted by swap operations, their starting execution time can be misaligned in subsequent search rounds, leading to a lost of opportunities for grouped ion shift.

\begin{figure}[t!]
        \centering
        \includegraphics[width=\linewidth, trim=0.1in 0.4in 0.3in 0.2in, clip]{fig/group_shift.pdf}
        
        \caption{ }
        \label{fig:group_shift}
\end{figure}
\noindent \textbf{\textcolor{red}{1. Intra-Trap S3 Aggregation:}} For each 1D trap segment, we analyze the shift intentions of different ions and group them into S3 instructions if multiple ions intend to move in the same direction without conflict in source/destination. Specifically, for all qubits involved in 2Q gates over the next few timesteps, we calculate the heuristic cost of its movements in all possible directions and select the ones with the lowest costs. Whenever a shift is selected, we lock the position of its destination, freeing the position of its source so that they can be occupied by subsequent shift. After that, we collect the selected shifts with the same direction within each 1D segment and group them into S3 instructions.

% \noindent \textbf{2. Inter-Trap JT-SIMD Grouping:} We examine inter-segment routing needs and group ion transfers that match one of the 18 pre-defined JT-SIMD classes. This process includes spatial binning of eligible junction transfers and matching them to hardware-supported movement templates.


% \noindent \textbf{2. Inter-Trap JT-SIMD Grouping:}
% In the stage of inter-trap movement search, we examine the 18 pre-defined JT-SIMD instructions and choose the one with the lowest cost according to our heuristic function. Specifically, for each of the 18 global transportation (e.g., global down shift), we check each qubit involved in 2Q gates over the next few timesteps, determining whether the qubit should be moved by this operation (e.g., stay at its position or shift down) according to which leads to a lower cost. These lower costs of all involved qubit sums into a total score for this JT-SIMD instruction, which is used to determine the best choice among the 18 possible JT-SIMD instructions.

\noindent \textbf{2. Inter-Trap JT-SIMD Grouping:}
We examine inter-segment routing needs and produce 18 instructions in the pred-defined JT-SIMD classes.
Specifically, for each of the 18 possible global operation, we determine which ions to move based on their routing needs, then aggregate them into a JT-SIMD instruction. Taking the global down shift operation, one of the 18 global operations, as an example, we check each qubit involved in 2Q gates over the next few timesteps, comparing the cost of shifting it down with that of keeping it staying at the original position, adopting the decision with the lower cost. Then, the ions chosen to be down shifted will be aggregate into a single JT-SIMD instruction.

\noindent \textbf{5. Gate Zone-Aware Heuristic Function}

To effectively guide SIMD aggregation and movement scheduling, our compiler employs a gate zone-aware heuristic that integrates both spatial and temporal priorities. This heuristic prioritizes gates whose qubits are positioned favorably with respect to target gate zones and penalizes those with higher routing overhead. Specifically, it evaluates each gate in the front layer based on its distance to an assigned target gate zone, along with the relative distance between participating qubits. Reassignment of gate zones occurs only under excessive routing delays, ensuring computational scalability. To mitigate congestion, the heuristic also deprioritizes gates targeting overloaded gate zones.

Formally, the heuristic cost is given by:

\begin{equation}
H = \sum_{g \in F, \ g.\text{qubits} \notin E} \left( d_{\text{gz}}(g) + \alpha \cdot \mathbb{I}{\text{tg}}(g) \cdot d{\text{inter}}(g) \right)
\end{equation}

Here, $F$ denotes the set of ready gates in the dependency graph (the front layer), and $E$ is the set of qubits currently involved in in-flight operations. The function excludes gates that cannot be scheduled immediately. The term $d_{\text{gz}}(g)$ captures the distance from all gate qubits to their assigned target gate zone, while $d_{\text{inter}}(g)$ measures inter-qubit spacing for two-qubit gates. The indicator $\mathbb{I}_{\text{tg}}(g)$ activates the inter-qubit term only when applicable. The coefficient $\alpha$ balances routing compactness and gate zone locality.

Unlike traditional compilers---which are oblivious to gate zone availability and rely on sparse ion placement to avoid contention---our heuristic enables high-density layouts and efficient gate scheduling by dynamically optimizing both movement and gate placement.
\begin{figure*}[t!]
        \centering
        \includegraphics[width=\linewidth]{fig/jt_aggregation.pdf}
        
        \caption{ }
        \label{fig:jt_aggregation}
\end{figure*}
% \begin{figure}[!h]
%         \centering
%         \includegraphics[width=0.8\linewidth, trim=0.1in 0.2in 0.3in 0.2in, clip]{fig/2d_heuristic.pdf}

%         \caption{}
%         \label{fig:2d_heuristic}
% \end{figure}


\subsection{SIMD Scheduling Pass: Cost-Aware Global Instruction Planning}
Once SIMD instructions are formed, they must be scheduled under hardware constraints. A naive scheduling may introduce excessive junction contention, control overhead, or thermal violation. We therefore perform cost-aware planning across time steps.

At a high level, many SIMD instructions---whether intra-trap S3 or inter-trap JT-SIMD---enable ion movement that brings qubits closer together for upcoming two-qubit gates. However, only a subset of these instructions can be executed at any given time due to architectural constraints. The goal of this scheduling pass is to determine \emph{which} SIMD instructions to prioritize at each moment in time, so as to minimize total routing cost while maintaining gate readiness.



% \begin{figure}[!h]
%         \centering
%         \includegraphics[width=0.8\linewidth, trim=0.1in 0.2in 0.3in 0.2in, clip]{fig/2d_heuristic.pdf}

%         \caption{}
%         \label{fig:2d_heuristic}
% \end{figure}

\noindent \textbf{\textcolor{red}{1. Global JT-SIMD Class Selection:}} At each clock cycle, only one JT-SIMD class is allowed. Our scheduler uses a lookahead window to evaluate which JT-SIMD class enables the most progress in terms of ready-to-route ions. A priority queue ranks classes by aggregate ion distance reduction and alignment with future gates.

% As illustrated in Figure~\ref{fig:2d_heuristic}, the scheduler begins by identifying two candidate SIMD groups: a downright JT-SIMD shift involving ${Q_0, Q_4}$ and a rightward JT-SIMD shift involving ${Q_3}$. Based on their respective heuristic costs, the downright group provides more effective layout progress and is selected for execution. This movement brings $Q_0$ and $Q_4$ into gate zones, enabling the immediate execution of two-qubit gates $(Q_0, Q_1)$ and $(Q_4, Q_5)$. In the subsequent timestep, the scheduler evaluates available inter-trap classes again and opts for a horizontal JT-SIMD swap between $Q_0$ and $Q_3$, instead of continuing with the upright shift of $Q_3$. This decision is guided by the forward progress metric associated with gate $(Q_2, Q_3)$. Following an intra-trap swap between $Q_1$ and $Q_3$, the gate $(Q_2, Q_3)$ is successfully executed, demonstrating how the scheduler dynamically selects the most beneficial JT-SIMD class per cycle based on routing urgency and gate readiness.

% \noindent \textbf{1. Prioritizing Intra-Trap S3 over Inter-Trap JT-SIMD:} Since intra-trap movement is faster and thermally cheaper, our scheduler always attempts to schedule as many S3 instructions as possible before initiating inter-trap JT-SIMD movement.

\noindent \textbf{2. Intra-Trap S3 over Inter-Trap JT-SIMD Selection:} In trapped-ion systems, intra-trap and inter-trap SIMD instructions cannot be executed simultaneously due to hardware-level control restrictions. Moreover, inter-trap transport operations typically incur 2--3$\times$ higher latency and larger thermal overhead compared to intra-trap shifts. To effectively coordinate these movement types, our scheduler dynamically selects between intra-trap S3 and inter-trap JT-SIMD instructions by comparing their potential to reduce the overall heuristic cost.

At each scheduling step, the compiler evaluates two candidate transport plans: one composed purely of intra-trap S3 shifts, and another that includes inter-trap JT-SIMD instructions. The scheduler prioritizes intra-trap S3 instructions for their lower latency and less thermal overhead, while activating inter-trap JT-SIMD opportunistically to unlock critical inter-trap routing progress. Specifically, global inter-trap movement is initiated only when its benefit to routing significantly outweighs that of intra-trap alternatives. Let $\mathcal{H}(G, \pi)$ denote the current heuristic cost of the system layout, and let $\pi_{\text{intra}}$ and $\pi_{\text{inter}}$ represent the resulting qubit mappings after applying intra-trap and inter-trap transports, respectively, the condition of selecting inter-trap JT-SIMD can be expressed as:

\begin{equation}
\mathcal{H}(G, \pi) - \mathcal{H}(G, \pi_{\text{inter}}) > 2 \cdot (\mathcal{H}(G, \pi) - \mathcal{H}(G, \pi_{\text{intra}}))
\end{equation}

% This decision rule ensures that inter-trap movement is initiated only when its benefit to global routing significantly outweighs that of intra-trap alternatives. By default, the scheduler prioritizes intra-trap S3 instructions for their lower cost and thermal efficiency, while activating inter-trap JT-SIMD opportunistically to unlock critical long-distance routing progress.


% \noindent \textbf{3. Gate Zone-Aware Co-Scheduling:} The scheduler jointly considers movement and gate execution. It delays JT-SIMD operations that would place ions into over-congested gate zones, instead favoring temporally spaced routing.

% \noindent \textbf{4. Conflict Resolution and Reordering:} If multiple SIMD instructions conflict (e.g., overlapping destinations), a greedy reordering pass is applied to resolve the contention while preserving overall throughput.




% The separation of intra- and inter-trap movement search plays an important role due to the constraint that intra-trap and inter-trap SIMD instructions cannot be executed simultaneously. 

This decision rule naturally enables the aggregation of more inter-trap movements, thereby enhancing the movement efficiency.
Fig.~\ref{fig:jt_aggregation} demonstrates this benefit  with an example of implement a circuit in Fig.~\ref{fig:jt_aggregation}(a1) with an initial layout in Fig.~\ref{fig:jt_aggregation}(a2). Without this decision rule, compilers may eagerly execute JT-SIMD instructions once their cost is lower than S3 instructions. This would lead to an operation scheduling with the steps shown in Fig.~\ref{fig:jt_aggregation}(b1).
\textbf{Step 1:} the 2Q gate between Q2 and Q3 is first conducted as these two qubits are adjacent. Meanwhile, Q1 and Q3 can be brought closer by an intra-trap down shift on Q1, while Q4 and Q5 can be brought closer by an inter-down-right shift on Q4. Due to hardware constraints, the latter one is scheduled after the former one is complete, as shown in Fig.~\ref{fig:jt_aggregation}(b2). \textbf{Step 2:} The 2Q gate between Q4 and Q5 is conducted since the two qubits are adjacent now. Concurrently, Q1 and Q3 are brought further closer by further shifting down Q1 and 
swapping Q2 and Q3. \textbf{Step 3:} An inter-trap shift on Q1 is conducted to bring Q1 adjacent to Q3, so that the 2Q gate between Q1 and Q3 can be conducted now.
Taking the latency of each operation into account, this scheduling can be translated to that in Fig.~\ref{fig:jt_aggregation}(b2), leading to an overall computation time of $862\mu s$. Note that while the two inter-trap shifts are in the same direction, they are conducted separately due to the eager execution of JT-SIMD instructions.

In contrast, with the decision rule above, our compiler can provide an optimized scheduling that identifies and groups inter-trap movements along the same direction. With the same example, our compiler would schedule operations in the following steps, as represented by Fig.~\ref{fig:jt_aggregation}(c1). \textbf{Step~1:} The 2Q gate between Q2 and Q3 is first conducted as these qubits are adjacent. Concurrently, Q1 is shifted down for two steps to get closer to Q3. \textbf{Step 2:} Q2 and Q3 are swapped to bring Q3 closer to Q1. \textbf{Step 3:} Q1 and Q4 are shifted in the down-right direction by a global inter-trap transportation to bring them adjacent to Q3 and Q5, so that the two 2Q gates between Q1,Q3 and between Q4,Q5 can be conducted.
The primary optimization in these steps is that our compiler delays and groups the inter-trap shifts on Q1 and Q4 to reduce transportation latency. As shown in Fig.~\ref{fig:jt_aggregation}(c2), this reduces the overall computation time to $662\mu s$ only. 

% \noindent \textbf{3. Selection between Intra-trap S3 and JT-SIMD:} The switch between them is determined by a comparison of their heuristic costs. That is, at each scheduling step, the compiler evaluates two candidate transport plans: one composed purely of intra-trap S3 instructions, and another that includes inter-trap JT-SIMD instructions. As inter-trap movements typically incurs 2-3$\times$ higher latency and larger thermal overhead compared intra-trap movements, we prioritize the scheduling of intra-trap movement, switching to a JT-SIMD instruction only if the cost of the inter-trap plan is significantly lower than the intra-trap one.

% \noindent \textbf{3. Greedy Aggregation with Priority Heuristics:} When multiple grouping options are available (e.g., longer or wider SIMD candidates), we use a cost model based on estimated latency and interference to select the most profitable aggregation. Priorities are given to wider S3 groups and inter-trap movements that avoid congested junctions. \todo{a little confusing}

% \noindent \textbf{3. Fallback to Scalar Instructions:} Any movement that cannot be safely grouped is left as a traditional scalar movement instruction. These operations follow a standard routing procedure and are scheduled individually.

\noindent \textbf{3. Time-sliced SIMD Synchronization:} In a scheduling process, operations may complete at different times due to their distinct latencies, effectively dividing execution into fine-grained time slices. To improve scheduling within each time slice, we propose a synchronization mechanism that enhances scheduling precision and minimizes qubit idle time by tracking real-time execution information.

This mechanism handles three types of information at each time slice:
(1) Qubit usage — it tracks which qubits are engaged in operations and which are idle, preventing the scheduling of operations that require the currently engaged qubits.
(2) Position availability — it monitors which positions are occupied or free, enabling immediate scheduling of operations once space is freed by other operations.
(3) Program dependencies — it maintains a dynamic dependency graph for the program to identify executable operations as soon as their prerequisites complete.

% In a scheduling, the completion time of different operations can be misaligned due to the disparity in their latencies, thereby dividing time into fine-grained slices. To enable better scheduling at each time slice, we propose a synchronization mechanism that enhances scheduling precision and minimize qubit idle time by tracking real-time execution information.

% This synchronization tracks three types of real-time information in each fined-grained time slice. (1) It tracks which qubits are engaged in operations and which are idle, thereby avoiding scheduling operations that involve the engaged qubits. (2) It tracks which positions are available and which are occupied, thereby finding executable operations once a position is freed by other operations. (3) It tracks the dependency graph of the program, thereby identifying more executable operations once the operations they depend on are complete.
  

\begin{figure}[h!]
        \centering
        \includegraphics[width=\linewidth, trim=0.1in 0.2in 0.3in 0.2in, clip]{fig/time_sync.pdf}
        
        \caption{ }
        \label{fig:time_sync}
\end{figure}

The advantage of our fine-grained synchronization can be illustrated by an example in Fig.~\ref{fig:time_sync}, where the TI systems implements the circuit in Fig.~\ref{fig:time_sync}(a1) with an initial layout in Fig.~\ref{fig:time_sync}(a2). Without an awareness of latency disparity, compilers would employ a depth-oriented synchronization, with operations scheduled in the steps shown in Fig.~\ref{fig:time_sync}(b1). \textbf{Step 1:} The 1Q gate is conducted on Q4. Concurrently, Q1 and Q3 are brought adjacent by swapping Q1 with Q2. \textbf{Step 2:} The 2Q gate between Q1 and Q3 is conducted. Meanwhile, Q4 is shifted up to become adjacent to Q3 and Q5 is shifted up to get closer to Q3.
\textbf{Step 3:} The 2Q gate between Q3 and Q4 is conducted. \textbf{Step 4:} Q5 is brought adjacent to Q3 by swapping with Q4. \textbf{Step 5:} The 2Q gate between Q3 and Q5 is conducted. Taking the latency of each operation into account, this scheduling can be translated to that in Fig.~\ref{fig:time_sync}(b2), leading to an overall computation time of $823\mu s$.


In contrast, with the time-sliced synchronization, our compiler can produce a better scheduling as shown in \ref{fig:time_sync}(c1), which has the following steps. \textbf{Step 1:} The 1Q gate is conducted on Q4, while Q1 and Q3 are brought adjacent by swapping Q1 with Q2. \textbf{Step 2:} A grouped shift is conducted on Q4 and Q5 in the up direction to bring them closer to Q3. \textbf{Step 3:} The 2Q
gate between Q3 and Q4 is conducted, considering that the swap gate between Q1 and Q2 is still executing. \textbf{Step 4:} After the 2Q gate between Q3 and Q4 is completed, we then swap Q4 and Q5 to bring Q4 adjacent to Q3, and conduct the 2Q gate between Q1 and Q3. \textbf{Step 5:} This is followed by the 2Q gate between Q3 and Q5. 

The main difference between our scheduling and the depth-oriented scheduling is that we fill up the time of the swap operation between Q1 and Q2 with the execution of 2Q gate between Q3 and Q4. We remark that this cannot be identified by compilers with a depth-oriented synchronization, despite that the 2Q gate between Q1 and Q3 and that between Q3 and Q4 are actually commutable. This is because as shown in \ref{fig:time_sync}(b1), they would think that the shift on Q4 has to be initiated after the completion of swap between Q1 and Q2, hence the 2Q gate cannot between Q3 and Q4 are not executable until the next depth. This forces the compiler to choose the 2Q gate between Q1 and Q3 in the current depth. Overall, our time-sliced synchronization leads to a shorter computation latency of $525\mu s$.


% \section{Simulation-based Scheduler}\label{sect:scheduler}

% \begin{algorithm}
% \caption{Compilation Process}
% \label{alg:scheduler}
% \SetKwFunction{dependency}{dependency\_graph}
% \SetKwFunction{intraschedule}{intra\_schedule}
% \SetKwFunction{interschedule}{inter\_schedule}
% \SetKwFunction{clearops}{clear\_ops}
% \SetKwFunction{update}{update}
% \SetKwFunction{Heur}{H}

% \KwData{Quantum circuit $C$, position graph $G$, initial mapping $\pi$ }
% \KwResult{Scheduled gate operations, execution time}
% $DG \leftarrow \dependency{C}$, $execution\_time \leftarrow 0$, $active\_ops \leftarrow \{\}$\;

% \SetKwProg{Fn}{Function}{:}{}
% \textit{\textbf{// remove completed operations from active\_ops and DG}}\\
% \Fn{\clearops{$active\_ops$, $T$}}{
%     \For{$op \in active\_ops$}{
%         $active\_ops[op] \leftarrow active\_ops[op] - T$\;
        
%         \If{$active\_ops[op] \leq 0$}{
         
%         del $active\_ops[op]$\;
        
%         $DG.F.remove(op)$\;}
%     }
% }

% \While{DG.F and active\_ops not empty}{
%     $execute\_ops, wait\_ops \leftarrow \emptyset$\;
%     $inter\_op\_flag \leftarrow False$\;
%     \textit{\textbf{// divide pending gates into executable and transport-required gates}}\\
%     \For{$g \in DG.F$}{
%         \If{$g$ is executable}{$execute\_ops.append(g)$}
%         \Else{$wait\_ops.append(g)$}
%     }

%     $\update{active\_ops, execute\_ops, $\pi$}$\;
%     ${\pi}_{intra}, intra\_ops \leftarrow \intraschedule{G, $\pi$, wait\_ops}$\;
%     ${\pi}_{inter}, inter\_ops \leftarrow \interschedule{G, $\pi$, wait\_ops}$\;

%     \textit{\textbf{// decision for adaptive inter/intra-trap switching}}\\
%     \If{2(\Heur{G, $\pi$} - \Heur{G, ${\pi}_{intra}$}) > \Heur{G, $\pi$} - \Heur{G, ${\pi}_{inter}$} }{
%         $inter\_op\_flag \leftarrow True$\;
%         \textit{\textbf{// update scheduler with LRT}}\\
%         $T \leftarrow LRT$\;
%     }
%     \Else{
%         $\update{active\_ops, intra\_ops, $\pi$}$\;
%         \textit{\textbf{// update scheduler with SRT}}\\
%         $T \leftarrow SRT$\;
%     }
    
%     $execution\_time += T$\;
%     \clearops{$active\_ops$, $T$}\;
%     \textit{\textbf{// execute inter-trap transport after clearing intra-trap transport in active\_ops}}\\
%     \If{inter\_op\_flag}{
%         $\update{active\_ops, inter\_ops, $\pi$}$\;
%         $T \leftarrow \min(active\_ops.values())$\;
%         $execution\_time += T$\;
%         \clearops{$active\_ops$, $T$}\;
%     }
% }
% \end{algorithm}

% This section introduces a scheduling framework that tackles two key challenges: time disparities between operations and execution conflicts between intra- and inter-trap operations. To address these issues, our framework incorporates (1) Real-Time Execution Tracking to enhance scheduling precision and minimize qubit idle time, and (2) Adaptive Inter/Intra-Trap Switching, a decision module that batches inter-trap transport to reduce costly context switching. By combining these strategies, our approach optimizes execution time and improves overall efficiency.



% \subsection{Real-Time Execution Tracking}\label{sect:real_time_tracking}

% The real-time execution tracking mechanism continuously tracks the quantum operations in execution and their remaining durations, enabling adaptive gate scheduling that can dynamically take advantage of optimal execution opportunities as they arise during circuit execution. By identifying which qubits are engaged in operations and which are idle, it allows the scheduler to prioritize certain operations while deferring others, effectively utilizing idle gaps in execution for additional tasks and optimizing overall circuit performance.

% The tracking process is focused on three key aspects:

% \begin{enumerate}
%     \item \textbf{Active Operation Tracking} - Monitors the operations currently being executed and their remaining durations in the active operations table ($active\_ops$), as described in Algorithm \ref{alg:scheduler}. It also identifies which qubits are involved in the execution. The shortest remaining time (SRT) in the table is then used to update the scheduler.
    
%     \item \textbf{Qubit Position and Space Tracking} - Tracks the real-time availability of empty spaces where qubits can be moved and the current position of each qubit, which includes both the trap number (indicating the trap the qubit is in) and the qubit's position within that trap.

%     \item \textbf{Dependency Graph Tracking} - Tracks updates to the dependency graph ($DG$), removing completed operations and marking dependent operations as pending, thereby creating a feedback loop between execution and scheduling.
% \end{enumerate}

% As shown in Algorithm \ref{alg:scheduler}, during each scheduling cycle, the scheduler examines all gates in the front layer of the dependency graph ($DG$), classifying them into two categories:  

% \begin{enumerate}
%     \item \textbf{Executable Gates}: Gates that can be executed immediately-for single-qubit gates with qubits in the computation zone and for two-qubit gates with both qubits in the same computation zone. These gates are added to the active operations table ($active\_ops$).  
%     \item \textbf{Gates Requiring Transport}: Gates whose qubits are not yet in the required locations. The scheduler schedules the necessary one-step transport operations to move the qubits and adds these operations to $active\_ops$.  
% \end{enumerate}

% The durations of all these newly-added operations in $active\_ops$ are updated based on hardware parameters in Table \ref{tab:hardware_data_table}. Simultaneously, $\pi$, which tracks qubit positions and available spaces, is updated to reflect changes due to intra- and inter-trap transport. At the end of each cycle, we assume a certain amount of time has passed, decrementing the remaining time for all active operations. Any operation with zero or less remaining time is considered complete and removed from $active\_ops$, triggering an update in $DG$ where completed operations are removed, and dependent gates are unlocked for scheduling in the next cycle.

% Generally, the time passed before the scheduler proceeds to the next cycle is set to the shortest remaining time (SRT) among the current active operations, as qubits and dependent tasks are only released upon the completion of the shortest task. This efficiently handles system changes in quantum computing, updating at task completion to optimize resource use without added too much overhead. More frequent updates would incur unnecessary costs without new information. Thus, SRT balances efficiency, simplicity, and reliability. Special cases exist, which will soon be discussed in Section \ref{sect:intra_vs_inter}.


% This comprehensive tracking mechanism ensures that the scheduler has up-to-date information to optimize the execution process and maximize resource utilization.


==> 05_tech.tex <==
% \section{Switchable Position Graph}\label{sect:position_graph}

% In contrast to traditional approaches that abstract the connectivity between qubits, we propose to abstract the connectivity between positions. In trapped-ion quantum computing, solely considering qubit-to-qubit connections fails to capture the availability of empty spaces between qubits. These empty positions are critical for scheduling shift operations efficiently. Furthermore, as qubits move, their connectivity dynamically changes, significantly increasing the complexity of compilation. By shifting the abstraction to position connectivity, we achieve a more stable representation that better facilitates transport scheduling.

% Additionally, we account for the constraint that, in a 2D trapped-ion system, transport operations can only proceed in one direction at a time. To handle inter-trap movement efficiently, we introduce an additional switching mechanism at the inter-trap level, ensuring that transport operations adhere to 2D directional constraints while maintaining efficient scheduling.

\section{SIMD }\label{sect:position_graph}  

% Unlike traditional methods that abstract qubit connectivity, we focus on position connectivity. In trapped-ion systems, considering only qubit-to-qubit connections overlooks empty positions, which are essential for shift operation scheduling. Additionally, qubit connectivity dynamically changes with transport, increasing compilation complexity. By modeling position connectivity, we achieve a stable representation that better supports transport scheduling.

% \subsection{Position Graph Construction}

% The position graph \( G(V, E) \) is derived from a QCCD hardware description, which specifies the \textbf{grid topology}—defining the abstract 2D hybrid system where nodes represent junctions and edges correspond to 1D traps—and the \textbf{1D trap capacity}, which dictates the number of contiguous positions per 1D trap, thus determining the granularity of qubit transport.

% The graph \( G(V, E) \) is defined as follows. The vertex set \( V \) consists of all valid positions, which are categorized into \textbf{gate zone positions} \( V_G \), shown with a yellow background in Figure \ref{fig:position_graph}(b), where two-qubit gates occur; \textbf{auxiliary positions} \( V_A \), shown with a light blue background in Figure \ref{fig:position_graph}(b), used for storage and transport; and \textbf{junction porting positions} \( V_J \), which serve as interfaces for inter-trap transport at junctions. Each position in \( V \) is associated with information regarding whether it is occupied (represented by a solid green point) or contains empty space (represented by a transparent point). This information is essential for managing the initial qubit layout, which determines the starting configuration of qubits across the system.

% The edge set \( E \) encodes valid transport paths, including intra-trap swaps/shifts and inter-trap operations. Within a 1D trap, qubits perform neighboring swaps, one-step shifts, and two-qubit gates when co-located in \( V_G \), forming a linear topology (green line). At junctions, \( V_J \) provides all-to-all connectivity (gray line) within the junction itself, meaning qubit transport can occur between any connected porting positions. However, these transports are subject to specific constraints governing inter-trap movement. To enforce these constraints and ensure coherent scheduling, we further introduce a higher-level switching abstraction that regulates transport execution across the system.


% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=1\linewidth, trim=0.3in 0.3in 0in 0.1in, clip]{fig/position_graph.pdf}
%     \caption{}
%     \label{fig:position_graph}
% \end{figure}

% \subsection{Hierarchical Switching Mechanism}

% To better understand the constraints governing transport execution, we introduce a higher-level switching abstraction that conceptualizes the permissible transport operations at any given time. This abstraction reflects the fundamental restrictions that intra-trap and inter-trap transport cannot occur simultaneously, and hybrid inter-trap or mixed-direction transport is prohibited. In this abstraction, we introduce a directional switch, where in some cases the switch is inactive. The control of the switch is applied globally to the junction, ensuring that all operations within the junction comply with the same set of constraints. For inter-trap shift operations, the switch is represented as a unidirectional arrow, as indicated in Figure \ref{fig:position_graph}(c), signaling that the operation can only proceed in one direction. For inter-trap swap operations, it is represented as a bidirectional arrow, allowing exchange between two positions in both directions. This directional switching mechanism ensures that transport operations follow system-level constraints and avoids conflicts between operations. The decision-making process for managing the switch is discussed in more detail in Section \ref{sect:intra_vs_inter}.
 
Unlike traditional methods that abstract \textbf{qubit connectivity}, we focus on \textbf{position connectivity}. Conventional approaches typically model only data qubits as graph nodes, assuming empty positions can be traversed freely. However, in trapped-ion systems, empty positions are not merely passive spaces but critical resources that directly affect shift scheduling and gate execution feasibility. 
\textcolor{red}{(Jens: I find that the previous two sentences are unreadable at this point in the paper.)}
Additionally, qubit connectivity dynamically changes due to transport operations, increasing compilation complexity. By modeling position connectivity rather than just qubit connectivity, we achieve a stable representation that explicitly accounts for the role of empty positions, facilitating more efficient transport scheduling.
By applying global switch control, our approach prevents conflicting transport operations and ensures system-wide synchronization.

% \subsection{Position Graph Construction}

The Position Graph \( G(V, E) \) is derived from a QCCD hardware description, which defines the \textbf{grid topology}—specifying the abstract 2D hybrid system where nodes represent junctions and edges correspond to 1D traps—and the \textbf{1D trap capacity}, which dictates the number of contiguous positions per 1D trap, thus determining the granularity of qubit transport.
Unlike traditional qubit coupling graphs that only consider qubit-to-qubit connections, the Position Graph treats every valid position—occupied or vacant—as a graph vertex. 

The vertex set \( V \) is categorized into:  
(1) \textbf{Gate zone positions} \( V_G \) (yellow background in Figure~\ref{fig:position_graph}(b)), where two-qubit gates are executed;
(2) \textbf{Auxiliary positions} \( V_A \) (light blue background in Figure~\ref{fig:position_graph}(b)), used for storage and transport;
(3) \textbf{Junction porting positions} \( V_J \), serving as interfaces for inter-trap transport. Each position explicitly records whether it is \textbf{occupied} (solid green point) or \textbf{vacant} (transparent point), which is critical for managing shift feasibility and optimizing qubit layout. The Position Graph fundamentally differs from traditional qubit coupling graphs by making vacant space an active part of the connectivity model, ensuring transport planning integrates available resources effectively.

The edge set \( E \) encodes valid transport paths, including intra-trap swaps/shifts and inter-trap operations. Within a 1D trap, qubits perform neighboring swaps, one-step shifts, and two-qubit gates when co-located in \( V_G \), forming a linear topology (green line). At junctions, \( V_J \) provides all-to-all connectivity (gray line), meaning transport can occur between any connected porting positions.
Each inter-trap edge can explicitly show whether it is in use:
a unidirectional arrow (Fig.~\ref{fig:position_graph}(c)) denotes a shift, which is movement in one direction, while a bidirectional arrow indicates a swap, which is a two-way exchange.
Those inter-trap edges help us model a hardware constraint: only a single type of inter-trap operation (shift or swap) can execute system-wide.
\textcolor{red}{(Jens: the previous sentence seems inaccurate; it says something different than the constraint listed at the beginning of Section 6.2.)}

%% Jens: I moved the following text to the next subsection.
% However, inter-trap transports are subject to specific constraints. To enforce these constraints and ensure coherent scheduling, we further introduce a global switching mechanism that regulates transport execution across the system.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\linewidth, trim=0.3in 0.3in 0in 0.1in, clip]{fig/position_graph.pdf}
    \caption{\textcolor{red}{(Jens: in diagram (c), I think ``No Inter-Trap'' is misleading; I suggest ``No Shift/Swap''.)}}
    \label{fig:position_graph}
\end{figure}

%% \subsection{Hierarchical Switching Mechanism} 

% \textcolor{red}{(Jens: no text in this subsection justifies why the subsection header has the word ``Hierarchical''.  The rest of the paper uses ``Hierarchical'' rather little.  Perhaps replace ``Hierarchical'' with ``Global''.)}

% Inter-trap transports are subject to system constraints, which we enforce via a global switching mechanism that regulates transport execution across the system.  Specifically, this mechanism governs when and how inter-trap transport occurs, ensuring that scheduling remains consistent with hardware limitations.

% Inter-trap transports are subject to specific constraints. To enforce these constraints and ensure coherent scheduling, we further introduce a global switching mechanism that regulates transport execution across the system.
% To ensure transport operations adhere to system constraints, we introduce a global junction switch control mechanism. This mechanism governs when and how inter-trap transport occurs, ensuring that scheduling remains consistent with hardware limitations.

% The global switch operates as follows: If the schedule is sequentially determined, the switch originally remains inactive. When an inter-trap transport occurs, the switch activates, enforcing a global constraint: only one type of inter-trap operation (shift or swap) executes in a single direction system-wide.
% \textcolor{red}{(Jens: what does ``sequentially determined'' mean?)}


% By applying global switch control, our approach prevents conflicting transport operations and ensures system-wide synchronization. The decision-making process in our optimized solution for efficiently managing the switch is further detailed in Section~\ref{sect:intra_vs_inter}.

% \textcolor{red}{(Jens: seems to me that Section 4.2 is trying to do two things at the same time, namely (1) explain that only one type of inter-trap operation (shift or swap) executes in a single direction system-wide, and (2) give a preview of Section 6.  I think you should integrate (1) into Section 4.1 and move the rest of the text somewhere else, or delete it if it is redundant.}

\section{Step-by-step Heuristic Router}\label{sect:heuristic_router}

This section introduces a spatial-aware heuristic routing approach designed to optimize qubit transport scheduling. The heuristic function \( H \) prioritizes qubit proximity to the gate zone and resolves congestion through a gate priority mechanism. We detail routing strategies for intra-trap and inter-trap operations, focusing on efficient shift and swap scheduling. This approach improves quantum circuit execution efficiency by optimizing transport operations and minimizing delays.

\subsection{Spatial-Aware Heuristic Function}\label{sect:heuristic_function}

% To optimize the selection of the next step in the transport operation, we design a spatial-aware heuristic function, \( H \), which evaluates the resulting qubit layout after one-step transport. By comparing the values of \( H \), we determine the next transport step, ensuring efficient scheduling of transport operations. The function \( H \) takes into account the proximity of qubits to the gate zone as the dominant factor, along with the distance between the qubits involved in a gate. To further alleviate potential congestion when qubits compete for the gate zone, we incorporate a gate priority-based mechanism, which streamlines access and prevents conflicts.

To optimize transport scheduling, we design a spatial-aware heuristic function, \( H \), which evaluates qubit layout changes after a one-step transport. By comparing \( H \) values, we determine the next transport step, prioritizing qubit proximity to the gate zone. To further alleviate potential congestion when qubits compete for the gate zone, we incorporate a gate priority-based mechanism, which streamlines access and prevents conflicts.

\noindent \textbf{Heuristic Function.}
The heuristic function is shown below:
\begin{equation}
    H = \sum_{g \in F, \ g.\text{qubits} \notin E} \left( d_{\text{gz}}(g) + \alpha \cdot \mathbb{I}_{\text{tg}}(g) \cdot d_{\text{inter}}(g) \right)
\end{equation}

In this function, \(F\) represents the front layer of the gate dependency graph, which includes all the gates pending to be executed, provided that the qubits are positioned correctly in the hardware. \(E\) refers to the set of qubits that are currently involved in ongoing operations. The condition \(g.\text{qubits} \notin E\) ensures that we do not prioritize gates where the qubits are already engaged in another operation, preventing us from considering gates that cannot be executed in real-time.

The term \(d_{\text{gz}}(g)\) represents the distance from all qubits involved in a gate to a target gate zone. To optimize search time, this specific gate zone is generally calculated only once. For single-qubit gates, it refers to the closest qubit gate zone to the qubit, and for two-qubit gates, it refers to the closest gate zone to both qubits. If a gate zone becomes too "popular" (i.e., too many qubits are competing for it), we make adjustments when selecting the target gate zone. Additionally, if a gate fails to route successfully within a reasonable time frame, we re-evaluate the choice of the target gate zone. The term \(d_{\text{inter}}(g)\) applies only to two-qubit gates, encouraging qubits to be as close as possible within their gate zones. As a secondary objective, the weighting factor \(\alpha\) is typically set to a small value, such as 0.3, to prevent it from dominating the heuristic. In FTQC (Fault-Tolerant Quantum Computing), the heuristic function differentiates between Clifford and T gates. For T gates, the function includes an additional term \( d_{\text{mg}}(g) \), representing the distance to the magic state factory. For Clifford gates, it uses \( d_{\text{gz}}(g) \), which measures proximity to the gate zone. This distinction optimizes routing for both gate types in FTQC scenarios.


\noindent \textbf{Congestion Mitigation:}  
When multiple qubits attempt to access the same gate zone simultaneously, congestion may still arise, leading to deadlocks in execution. To avoid congestion, our heuristic function prioritizes gates based on the order in which their qubits were added to the routing process. This ensures that gates with earlier pending qubits are considered first, minimizing the risk of deadlocks and resolving conflicts efficiently.

\subsection{Intra-Trap and Inter-Trap Routing}\label{sect:trap-routing}

In both intra-trap and inter-trap routing, operations are scheduled separately since they cannot be executed simultaneously. Strategic scheduling is employed to ensure efficient qubit transport while avoiding conflicts and delays in gate execution. The decision of which routing type to prioritize is later discussed in section \ref{sect:intra_vs_inter}.

\noindent \textbf{Intra-trap routing.}
In intra-trap routing, we prioritize shift operations over swaps. Shift operations are scheduled in batches to optimize the use of available space in the trap. Before moving qubits, we ensure that the target space is free and not designated for another qubit's movement, avoiding conflicts. Additionally, we check that the selected qubits for shift and swap operations don't overlap with qubits already engaged in other tasks, ensuring smooth routing and preventing interference.

\noindent \textbf{Inter-trap routing.}
In inter-trap routing, we systematically collect transport operations and use a heuristic function to evaluate all possible directions for inter-trap shifts and swaps. Since operations in different directions can’t be executed at the same time, we consider each operation one by one. The heuristic function assigns a score to each direction, and after calculating the scores for all options, we choose the operations with the lowest total score. This set of operations forms a conflict-free transport schedule.

As shown in Figure \ref{fig:2d_heuristic}, the first scheduling step identifies two non-empty transport groups: a downright shift group ${Q_0, Q_4}$ and a right shift group ${Q_3}$. Since the first group has a lower score, the scheduler selects it to execute first, resulting in the successful execution of the two-qubit gates $(Q_0, Q_1)$ and $(Q_4, Q_5)$. In the next step, the scheduler opts to perform an inter-trap horizontal swap ${(Q_0, Q_3)}$ instead of the inter-trap upright shift ${Q_3}$. After an intra-trap swap between $Q_1$ and $Q_3$, the two-qubit gate $(Q_2, Q_3)$ is successfully executed.

By following this approach, the routing process is made efficient, ensuring that larger transport groups are handled without unnecessary detours. Ignoring the heuristic function could lead to suboptimal routing, splitting of larger groups, and delays in gate execution.


\begin{figure}[!h]
        \centering
        \includegraphics[width=0.8\linewidth, trim=0.1in 0.2in 0.3in 0.2in, clip]{fig/2d_heuristic.pdf}

        \caption{}
        \label{fig:2d_heuristic}
\end{figure}

\section{Simulation-based Scheduler}\label{sect:scheduler}

\begin{algorithm}
\caption{Compilation Process}
\label{alg:scheduler}
\SetKwFunction{dependency}{dependency\_graph}
\SetKwFunction{intraschedule}{intra\_schedule}
\SetKwFunction{interschedule}{inter\_schedule}
\SetKwFunction{clearops}{clear\_ops}
\SetKwFunction{update}{update}
\SetKwFunction{Heur}{H}

\KwData{Quantum circuit $C$, position graph $G$, initial mapping $\pi$ }
\KwResult{Scheduled gate operations, execution time}
$DG \leftarrow \dependency{C}$, $execution\_time \leftarrow 0$, $active\_ops \leftarrow \{\}$\;

\SetKwProg{Fn}{Function}{:}{}
\textit{\textbf{// remove completed operations from active\_ops and DG}}\\
\Fn{\clearops{$active\_ops$, $T$}}{
    \For{$op \in active\_ops$}{
        $active\_ops[op] \leftarrow active\_ops[op] - T$\;
        
        \If{$active\_ops[op] \leq 0$}{
         
        del $active\_ops[op]$\;
        
        $DG.F.remove(op)$\;}
    }
}

\While{DG.F and active\_ops not empty}{
    $execute\_ops, wait\_ops \leftarrow \emptyset$\;
    $inter\_op\_flag \leftarrow False$\;
    \textit{\textbf{// divide pending gates into executable and transport-required gates}}\\
    \For{$g \in DG.F$}{
        \If{$g$ is executable}{$execute\_ops.append(g)$}
        \Else{$wait\_ops.append(g)$}
    }

    $\update{active\_ops, execute\_ops, $\pi$}$\;
    ${\pi}_{intra}, intra\_ops \leftarrow \intraschedule{G, $\pi$, wait\_ops}$\;
    ${\pi}_{inter}, inter\_ops \leftarrow \interschedule{G, $\pi$, wait\_ops}$\;

    \textit{\textbf{// decision for adaptive inter/intra-trap switching}}\\
    \If{2(\Heur{G, $\pi$} - \Heur{G, ${\pi}_{intra}$}) > \Heur{G, $\pi$} - \Heur{G, ${\pi}_{inter}$} }{
        $inter\_op\_flag \leftarrow True$\;
        \textit{\textbf{// update scheduler with LRT}}\\
        $T \leftarrow LRT$\;
    }
    \Else{
        $\update{active\_ops, intra\_ops, $\pi$}$\;
        \textit{\textbf{// update scheduler with SRT}}\\
        $T \leftarrow SRT$\;
    }
    
    $execution\_time += T$\;
    \clearops{$active\_ops$, $T$}\;
    \textit{\textbf{// execute inter-trap transport after clearing intra-trap transport in active\_ops}}\\
    \If{inter\_op\_flag}{
        $\update{active\_ops, inter\_ops, $\pi$}$\;
        $T \leftarrow \min(active\_ops.values())$\;
        $execution\_time += T$\;
        \clearops{$active\_ops$, $T$}\;
    }
}
\end{algorithm}

This section introduces a scheduling framework that tackles two key challenges: time disparities between operations and execution conflicts between intra- and inter-trap operations. To address these issues, our framework incorporates (1) Real-Time Execution Tracking to enhance scheduling precision and minimize qubit idle time, and (2) Adaptive Inter/Intra-Trap Switching, a decision module that batches inter-trap transport to reduce costly context switching. By combining these strategies, our approach optimizes execution time and improves overall efficiency.



\subsection{Real-Time Execution Tracking}\label{sect:real_time_tracking}

The real-time execution tracking mechanism continuously tracks the quantum operations in execution and their remaining durations, enabling adaptive gate scheduling that can dynamically take advantage of optimal execution opportunities as they arise during circuit execution. By identifying which qubits are engaged in operations and which are idle, it allows the scheduler to prioritize certain operations while deferring others, effectively utilizing idle gaps in execution for additional tasks and optimizing overall circuit performance.

The tracking process is focused on three key aspects:

\begin{enumerate}
    \item \textbf{Active Operation Tracking} - Monitors the operations currently being executed and their remaining durations in the active operations table ($active\_ops$), as described in Algorithm \ref{alg:scheduler}. It also identifies which qubits are involved in the execution. The shortest remaining time (SRT) in the table is then used to update the scheduler.
    
    \item \textbf{Qubit Position and Space Tracking} - Tracks the real-time availability of empty spaces where qubits can be moved and the current position of each qubit, which includes both the trap number (indicating the trap the qubit is in) and the qubit's position within that trap.

    \item \textbf{Dependency Graph Tracking} - Tracks updates to the dependency graph ($DG$), removing completed operations and marking dependent operations as pending, thereby creating a feedback loop between execution and scheduling.
\end{enumerate}

As shown in Algorithm \ref{alg:scheduler}, during each scheduling cycle, the scheduler examines all gates in the front layer of the dependency graph ($DG$), classifying them into two categories:  

\begin{enumerate}
    \item \textbf{Executable Gates}: Gates that can be executed immediately-for single-qubit gates with qubits in the computation zone and for two-qubit gates with both qubits in the same computation zone. These gates are added to the active operations table ($active\_ops$).  
    \item \textbf{Gates Requiring Transport}: Gates whose qubits are not yet in the required locations. The scheduler schedules the necessary one-step transport operations to move the qubits and adds these operations to $active\_ops$.  
\end{enumerate}

The durations of all these newly-added operations in $active\_ops$ are updated based on hardware parameters in Table \ref{tab:hardware_data_table}. Simultaneously, $\pi$, which tracks qubit positions and available spaces, is updated to reflect changes due to intra- and inter-trap transport. At the end of each cycle, we assume a certain amount of time has passed, decrementing the remaining time for all active operations. Any operation with zero or less remaining time is considered complete and removed from $active\_ops$, triggering an update in $DG$ where completed operations are removed, and dependent gates are unlocked for scheduling in the next cycle.

Generally, the time passed before the scheduler proceeds to the next cycle is set to the shortest remaining time (SRT) among the current active operations, as qubits and dependent tasks are only released upon the completion of the shortest task. This efficiently handles system changes in quantum computing, updating at task completion to optimize resource use without added too much overhead. More frequent updates would incur unnecessary costs without new information. Thus, SRT balances efficiency, simplicity, and reliability. Special cases exist, which will soon be discussed in Section \ref{sect:intra_vs_inter}.


This comprehensive tracking mechanism ensures that the scheduler has up-to-date information to optimize the execution process and maximize resource utilization.


\subsection{Adaptive Inter/Intra-Trap Switching}\label{sect:intra_vs_inter}
In a trapped-ion quantum system, inter-trap and intra-trap transport operations cannot be executed simultaneously due to hardware constraints, necessitating an effective coordination mechanism for switching between them. Additionally, inter-trap transport operations typically take 2–3 times longer than intra-trap transport operations. As a result, the scheduling strategy generally prioritizes intra-trap transport to maximize local efficiency, while inter-trap transport operations accumulate before being executed in batches to amortize their higher cost.

To effectively manage this trade-off, we introduce the \textit{Adaptive Inter/Intra-Trap Switching} mechanism, which dynamically selects the optimal transport strategy based on the qubit mapping quality. This mechanism leverages the heuristic function $\mathcal{H}$ described in Section \ref{sect:heuristic_router} to evaluate two potential paths: \textbf{Intra-trap}, which updates the qubit mapping by adjusting qubits' local positions within the same trap while executing only local operations, and \textbf{Inter-trap}, which modifies the qubit mapping by relocating qubits across traps in addition to adjusting their local positions. The decision criterion is formulated as:

\[
\mathcal{H}(G, \pi) - \mathcal{H}(G, \pi_{\text{inter}})  > 2(\mathcal{H}(G, \pi) - \mathcal{H}(G, \pi_{\text{intra}}))
\]

where $\pi_{\text{inter}}$ and $\pi_{\text{intra}}$ represent the post-scheduling qubit mappings for the inter-trap and intra-trap strategies, respectively. The scheduling decision follows the criterion that inter-trap transport is prioritized when the reduction in heuristic cost achieved by inter-trap transport is more than twice the reduction achieved by intra-trap transport. Otherwise, intra-trap operations continue to be executed. 

After making the switching decision, the system updates the scheduler differently depending on the selected transport type. If the intra-trap transport operations are chosen, the scheduler follows the shortest remaining time (SRT) strategy, as described in Section \ref{sect:real_time_tracking}. In contrast, if an inter-trap transport operation is selected, the scheduler adopts the longest remaining time (LRT) strategy, meaning that all remaining intra-trap operations in the active operations table are first cleared before executing the inter-trap operations. This adaptive approach ensures a balanced trade-off between local parallelism and global communication, improving overall execution efficiency within the given hardware constraints.

==> 07_secondary_table.tex <==
\begin{table}[h]
    \centering
    \caption{Results of our compiler when $D_f=1$ and the baseline. Each `benchmark-$n$' corresponds to an $n$-qubit circuit in the circuit model
    % , compiled to a 2D size of $\sqrt{n}\times\sqrt{n}$.
    }
  %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
    \resizebox{\linewidth}{!}{
        \renewcommand*{\arraystretch}{1}
        \begin{small}
            \begin{tabular}{|p{1.4cm}|p{1cm}|p{0.9cm}|p{0.7cm}|p{1.2cm}|p{1.1cm}|}
        
        \hline
        Benchmark - \#Qubit  & Qiskit Depth & Qiskit + Skew Depth & Our Depth & Depth Improv.  vs Qiskit  & Depth Improv. vs Qiskit + Skew\\ \hline
        QAOA-36 & 1,055 & 739 & 264 & 4.0 & 2.8 \\\hline
        QFT-36 & 2,063 & 1,164 & 507 & 4.07 & 2.3 \\\hline
        RCA-36 & 2,379 & 1,660 & 561 & 4.24 & 2.96 \\\hline
        VQE-36 & 830 & 367 & 191 & 4.35 & 1.92 \\\hline
        QAOA-64 & 3,279 & 1,810 & 557 & 5.89 & 3.25 \\\hline
        QFT-64 & 6,385 & 2,958 & 1,004 & 6.36 & 2.95 \\\hline
        RCA-64 & 4,397 & 2,994 & 1,075 & 4.09 & 2.79 \\\hline
        VQE-64 & 1,929 & 914 & 452 & 4.27 & 2.02 \\\hline
        QAOA-100 & 6,089 & 3,297 & 1,048 & 5.81 & 3.15 \\\hline
        QFT-100 & 9,206 & 7,945 & 1,798 & 5.12 & 4.42 \\\hline
        RCA-100 & 6,896 & 4,806 & 1,595 & 4.32 & 3.01 \\\hline
        VQE-100 & 4,723 & 1,780 & 813 & 5.81 & 2.19 \\\hline

    
    
    
    
                
    \end{tabular}
    \end{small}
    }
    \label{tab:secondary_table}
\end{table}

% \begin{table}[h]
%     \centering
%     \caption{}
%   %  The name column are acronyms of test programs in Table~\ref{tab:benchmark}.}
%     \resizebox{0.48\textwidth}{!}{
%         \renewcommand*{\arraystretch}{1.0}
%         \begin{footnotesize}
%             \begin{tabular}{|p{1.2cm}|p{1cm}|p{1cm}|p{0.7cm}|p{1.2cm}|p{1.6cm}|}
        
%         \hline
%         Benchmark - \#Qubit  & Braiding Depth & Non-Braiding Depth\\ \hline
%         QAOA-36 & 1,055 & 739 & 1.43 & 320 & 3.3 \\\hline
%         QFT-36 & 2,063 & 1,164 & 1.77 & 571 & 3.61 \\\hline
%         RCA-36 & 2,379 & 1,660 & 1.43 & 1,246 & 1.91 \\\hline
%         VQE-36 & 830 & 367 & 2.26 & 233 & 3.56 \\\hline
%         QAOA-49 & 1,982 & 971 & 2.04 & 479 & 4.14 \\\hline
%         QFT-49 & 2,615 & 1,877 & 1.39 & 861 & 3.04 \\\hline
%         RCA-49 & 3,272 & 2,277 & 1.44 & 1,741 & 1.88 \\\hline
%         VQE-49 & 1,834 & 678 & 2.71 & 349 & 5.26 \\\hline
%         QAOA-64 & 3,279 & 1,810 & 1.81 & 676 & 4.85 \\\hline
%         QFT-64 & 6,385 & 2,958 & 2.16 & 1,215 & 5.26 \\\hline
%         RCA-64 & 4,397 & 2,994 & 1.47 & 2,376 & 1.85 \\\hline
%         VQE-64 & 1,929 & 914 & 2.11 & 551 & 3.5 \\\hline
                
%     \end{tabular}
%     \end{footnotesize}
%     }
%     \label{tab:secondary_table}
% \end{table}
